Marvels and Pitfalls of the Langevin Algorithm in Noisy High-dimensional Inference

Gradient-descent-based algorithms and their stochastic versions have widespread applications in machine learning and statistical inference. In this work we perform an analytic study of the performances of one of them, the Langevin algorithm, in the context of noisy high-dimensional inference. We employ the Langevin algorithm to sample the posterior probability measure for the spiked matrix-tensor model. The typical behaviour of this algorithm is described by a system of integro-differential equations that we call the Langevin state evolution, whose solution is compared with the one of the state evolution of approximate message passing (AMP). Our results show that, remarkably, the algorithmic threshold of the Langevin algorithm is sub-optimal with respect to the one given by AMP. We conjecture this phenomenon to be due to the residual glassiness present in that region of parameters. Finally we show how a landscape-annealing protocol, that uses the Langevin algorithm but violate the Bayes-optimality condition, can approach the performance of AMP.

==> supplementary_content.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Definition of the spiked matrix-tensor model}\label{sec:model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We consider a teacher-student setting in which the teacher constructs a matrix and a tensor from a randomly sampled signal and the student is asked to recover the signal from the observation of the matrix and tensor provided by the teacher \cite{REVIEWFLOANDLENKA}.

The signal, $x^*$ is an $N$-dimensional vector whose entries are real i.i.d. random variables sampled from the normal distribution (i.e. the prior is $P_X\sim\mathcal{N}(0,1)$). 
The teacher generates from the signal a symmetric matrix and a symmetric tensor of order $p$.
Those two objects are then transmitted through two noisy channels with variances $\Delta_2$ and $\Delta_p$,
so that at the end one has two noisy observations given by
\begin{align}\label{eq:channel Y}
    & Y_{ij} = \frac{x_i^{*}x_j^*}{\sqrt{N}}+\xi_{ij},\\
    \label{eq:channel T}
    & T_{i_1,\dots,i_p} = \frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i_1}^*\dots x_{i_p}^*+\xi_{i_1,\dots,i_p},
\end{align}
where, for $i< j$ and $i_1< \dots < i_p$,  $\xi_{ij}$ and
$\xi_{i_1,\dots,i_p} $ are i.i.d. random variables distributed
according to $\xi_{ij}\sim {\cal N}(0,\Delta_2)$ and
$\xi_{i_1,\dots,i_p}\sim {\cal N} (0,\Delta_p)$. The $\xi_{ij}$ and
$\xi_{i_1,\dots,i_p}$ are symmetric random matrix and tensor,
respectively. 
Given $Y_{ij}$ and $T_{i_1,\dots,i_p}$ the inference task is to reconstruct the signal $x^*$. 

In order to solve this problem we consider the Bayesian approach.
This starts from the assumption that both the matrix and tensor have been produced from a process of the same kind of the one described by Eq.~(\ref{eq:channel Y}-\ref{eq:channel T}).
Furthermore we assume to know the statistical properties of the
channel, namely the two variances $\Delta_2$ and $\Delta_p$, and the
prior on $x$.
Given this, the posterior probability distribution over the signal is obtained through the Bayes formula
\begin{equation}
P(X|Y,T) = \frac{P(Y,T|X)P(X)}{P(Y,T)}\, , 
\end{equation}
where
\begin{equation} \label{eq:likelihood general}
    \begin{split}
        P(Y,T|X) &= \prod_{i< j}P_{Y}\left(Y_{ij}\Bigg|\frac{x_ix_j}{\sqrt{N}}\right)\prod_{ i_1<\dots<i_p}P_{T}\left(T_{i_1\dots i_p}\Bigg|\frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i_1}\dots x_{i_p}\right) =
        \\
        &\propto \prod_{i< j}e^{-\frac1{2\Delta_2}\left(Y_{ij}-\frac{x_ix_j}{\sqrt{N}}\right)^2}\prod_{ i_1<\dots<i_p}e^{-\frac1{2\Delta_p}\left(T_{i_1\dots i_p}-\frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i_1}\dots x_{i_p}\right)^2}.
    \end{split}
\end{equation}
Therefore we have 
 \begin{equation}\label{eq:posterior general}
    \begin{split}
        P(X|Y,T) &= \frac{1}{Z(Y,T)}\prod_{i}e^{-\frac12 x_i^2}\prod_{i< j}e^{-\frac1{2\Delta_2}\left(Y_{ij}-\frac{x_ix_j}{\sqrt{N}}\right)^2}\prod_{ i_1<\dots<i_p}e^{-\frac1{2\Delta_p}\left(T_{i_1\dots i_p}-\frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i_1}\dots x_{i_p}\right)^2},
    \end{split}
\end{equation}
where $Z(Y, T)$ is a normalization constant.

Plugging Eqs.~(\ref{eq:channel Y}-\ref{eq:channel T}) into
Eq.~(\ref{eq:posterior general}) allows to rewrite the posterior
measure in the form of a \emph{Boltzmann distribution} of the mixed $2+p$-spin Hamiltonian \cite{CL04, CL06, CL13}
\begin{equation}\label{eq:Hamiltonian}
	\begin{split}
		\mathcal{H} &= -\frac1{\Delta_2\sqrt{N}}\sum_{i<j}\xi_{ij}x_ix_j -\frac{\sqrt{(p-1)!}}{\Delta_pN^{\frac{p-1}2}}\sum_{i_1<\dots<i_p}\xi_{i_1\dots i_p}x_{i_1}\dots x_{i_p} - \frac{N}{2\Delta_2}\left(\frac1N\sum_ix_ix_i^*\right)^2 +\\
		& - \frac{N}{p\Delta_p}\left(\frac1N\sum_ix_ix_i^*\right)^p -\frac 12\sum_{i=1}^N x_i^2+ \text{const.}
	\end{split}
\end{equation}
so that
\begin{equation}
P(X|Y,T) = \frac{1}{\tilde Z(Y,T)} e^{- \mathcal{H}} \, . 
\label{Boltzmann}
\end{equation}
In the following we will refer to $\tilde Z(Y,T)$ as the \emph{partition function}.
We note here that in the large $N$ limit, using a Gaussian prior on the variables $x_i$ is
equivalent to consider a flat measure over the $N$-dimensional hypersphere $\sum_{i=1}^N x_i^2=N$. 
This choice will be used when we will describe the Langevin algorithm and in this case the last term in the Hamiltonian will become an irrelevant constant.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Approximate Message Passing, state evolution and phase diagrams}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Approximate Message Passing (AMP) is a powerful iterative algorithms to compute the local \emph{magnetizations} $\langle x_i\rangle$ given the observed matrix and tensor.
It is rooted in the cavity method of statistical physics of disordered
systems \cite{TAP77, MPV87} and it has been recently developed in the
context of statistical inference \cite{DMM09}, where in the Bayes optimal case it has been conjectured to be optimal among all local iterative algorithms. 
Among the properties that make AMP extremely useful is the fact that
its performances can be analyzed in the thermodynamic limit. Indeed in
such limit, its dynamical evolution is described by the so called
State Evolution (SE) equations \cite{DMM09}. 
In this section we derive the AMP equations and their SE description for the spiked matrix-tensor model and solve them to obtain the phase diagram of the model as a function of the variances $\Delta_2$ and $\Delta_p$ of the two noisy channels. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Approximate Message Passing and Bethe free entropy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:AMP}

AMP can be obtained as a relaxed Gaussian closure of the Belief Propagation (BP) algorithm. The derivation that we present follows the same lines of \cite{MiolaneTensor,LKZ17}. 
The posterior probability can be represented as a factor graph where all the variables are represented by circles and are linked to squares representing the interactions \cite{MM09}. 
\begin{figure}[H]
	\centering
	\includegraphics[scale=0.7]{img/figure_factor_graph/figura.pdf}
	\caption{The factor graph representation of the posterior
          measure of the matrix-tensor factorization model. The variable nodes represented with white
          circles are the components of the signal while black
          squares are factor nodes that denote interactions between
          the variable nodes that appear in the interaction
          terms of the Boltzmann distribution in Eqs.~(\ref{eq:Hamiltonian}-\ref{Boltzmann}). 
          There are three types of factor nodes: $P_X$ is the
          prior that depends on a single variable, $P_Y$ that is the
          probability of observing a matrix element $Y_{ij}$ given the
          values of the variables $x_i$ and $x_j$, and finally $P_T$
          that is the probability of observing a tensor element $T_{i_1,\dots,i_p}$. 
          The posterior, apart from the normalization factor, is simply given by the product of all the factor nodes.}  
\end{figure}
This representation is very convenient to write down the BP equations. In the BP algorithm we iteratively update until convergence a set of variables, which are beliefs of the (cavity) magnetization of the nodes. The intuitive underlying reasoning behind how BP works is the following. Given the current state of the variable nodes, take a factor node and exclude one node among its neighbors. The remaining neighbors through the factor node express a belief on the state of the excluded node. This belief is mathematically described by a probability distribution called \textit{message}, $\tilde{m}^t_{ij\rightarrow i}(x_i)$ and $\tilde{t}^t_{ii_2\dots i_p\rightarrow i}(x_i)$ depending on which factor node is selected. At the same time, another belief on the state of the excluded node is given by the rest of the network but the factor node previously taken into account, $m_{i\rightarrow ij}(x_i)$ and $t_{i\rightarrow ii_2\dots i_p}(x_i)$ respectively. All these \textit{messages} travel in the factor graph carrying partial information on the real magnetization of the single nodes, and they are iterated until convergence\footnote{Note that the pointwise convergence of the algorithm depends on the situations.}. The iterative scheme is described by the following equations
    \begin{align}
        \tilde{m}^{t}_{ij\rightarrow i}(x_i)&\propto\int dx_j m^t_{j\rightarrow ij}(x_j)P_Y\left(Y_{ij}\Bigg|\frac{x_ix_j}{\sqrt{N}}\right),\label{BP1}\\
        m^{t+1}_{i\rightarrow ij}(x_i)&\propto P_X(x_i)\prod_{l\neq j}
                                        \tilde{m}^t_{il\rightarrow
                                        i}(x_i)\prod_{i_2 < \dots
                                        <  i_p} \tilde{t}^t_{ii_2\dots i_p\rightarrow i}(x_i),\\
        \tilde{t}^{t}_{ii_2\dots i_p\rightarrow i}(x_i)&\propto\int
                                                       \prod_{l=2\dots
                                                       p}\left(dx_l
                                                       t^t_{i_l\rightarrow
                                                       ii_2\dots
                                                       i_p}(x_l)\right)
                                                       P_T\left(T_{ii_2\dots
                                                       i_p}\Bigg|\frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i}
                                                       x_{i_2}\dots
                                                       x_{i_p} \right),\\
        t^{t+1}_{i\rightarrow ii_2\dots i_p}(x_i)&\propto
                                                   P_X(x_i)\prod_{l}
                                                   \tilde{m}^t_{il\rightarrow
                                                   i}(x_i)\prod_{k_2
                                                   < \dots <
                                                   k_p\neq i_2\dots i_p} \tilde{t}^t_{ik_2\dots k_p\rightarrow i}(x_i)
                                                    \label{BP4}
    \end{align}
    and we have omitted the normalization constants that guarantee that the messages are probability distributions.
When the messages have converged to a fixed point, the estimation of the local magnetizations can be obtained through the computation of the real marginal probability distribution of the variables given by
\begin{equation}
\mu_i(x_i)=\int\left[\prod_{j(\neq i)}dx_j\right]
P(X|Y,T)=P_X(x_i)\prod_{l} \tilde{m}^t_{il\rightarrow
  i}(x_i)\prod_{i_2< \dots< i_p} \tilde{t}^t_{ii_2\dots
    i_p\rightarrow i}(x_i)\,. 
\end{equation}
We note that the computational cost to produce an iteration of BP  scales as $O(N^p)$. Furthermore Eqs.~(\ref{BP1} -\ref{BP4}) are iterative equations for continuous functions and therefore
are extremely hard to solve when dealing with continuous variables.
The advantage of AMP is to reduce drastically the computational
complexity of the algorithm by closing the equations on a Gaussian ansatz for the messages. 
This is justified in the present context since the factor graph is
fully connected and therefore each iteration step of the algorithm
involves sums of a large number of independent random variables that give rise to Gaussian distributions. 
Gaussian random variables are characterized by their mean and
covariance that are readily obtained for $N\gg 1$ expanding the factor nodes for small $\omega_{ij} =
x_i x_j   /  \sqrt{N}$ and $\omega_{i_1\dots i_p} =
\sqrt{(p-1)!} x_1 \dots x_p   / N^{\frac{p-1}2}$. 


Once the BP equations are relaxed on Gaussian messages, the final
 step to obtain the AMP algorithm is the so-called TAPyfication procedure \cite{LKZ17, TAP77},
which 
exploits the fact that the procedure of removing one node or one factor produces only a weak perturbation
to the real marginals and therefore can be described in terms of the real marginals of the variable nodes themselves.
By applying this scheme we obtain
the AMP equations, which are described by a set of auxiliary variables
$A^{(k)}$ and $B^{(k)}_i$ and by the mean $\langle x_i\rangle$ and variance $\sigma_i=\langle x_i^2\rangle$ of the marginals of variable nodes. 
%For Gaussian prior $P_x$ we have that the average of the variable $i$ over the posterior measure $\langle x_i\rangle$ is given by
%\begin{equation}
%	\hat{x}_i \doteq f(A,B) \equiv 
%        \int dx \frac1{{\cal Z}(A,B)}xP_X(x)e^{Bx-\frac12Ax^2} =
%\frac{B}{1+A},
%\end{equation} 
The AMP iterative equations are
    \begin{align}\label{eq:AMP B2}
        B^{(2),t}_{i}&=\frac{1}{\Delta_2\sqrt{N}}\sum_{k}Y_{ki}\hat{x}_k^t-\frac1{\Delta_2}\left(\frac1{N}\sum_k\sigma_k^t\right)\hat{x}_i^{t-1}\,;
        \\\label{eq:AMP A2}
        A^{(2),t}&=\frac{1}{\Delta_2 N}\sum_{k}\left(\hat{x}_k^t\right)^2\,;
        \\\label{eq:AMP Bp}
        B^{(p),t}_{i}&=\frac{\sqrt{(p-1)!}}{\Delta_p N^{(p-1)/2}}\sum_{k_2\dots k_p}T_{ik_2\dots k_p}\left(\hat{x}_{k_2}^t\dots \hat{x}_{k_p}^t\right)
        -\frac{p-1}{\Delta_p}\left[\left(\frac1{N}\sum_k\sigma_k^t\right)\;\left[\frac1{N}\sum_k
                       \hat{x}_k^t\hat{x}_k^{t-1}\right]^{p-2}\right]\hat{x}_i^{t-1}\,;
        \\\label{eq:AMP Ap}
        A^{(p),t}&=\frac1{\Delta_p}\left[\frac1{N}\sum_k\left(\hat{x}_k^t\right)^2\right]^{p-1}\,;
        \\\label{eq:AMP x}
        \hat{x}_i^{t+1}&=f(A^{(2)}+A^{(p)},B^{(2)}_i+B^{(p)}_i)\,;
        \\\label{eq:AMP sigma}
        \sigma_i^{t+1}&=\left.\frac{\partial}{\partial B}f(A,B)\right|_{A=A^{(2)}+A^{(p)},B=B^{(2)}_i+B^{(p)}_i}\,,\\
        f(A,B) &\equiv \int dx \frac1{{\cal Z}(A,B)}xP_X(x)e^{Bx-\frac12Ax^2} =\frac{B}{1+A}\:.
    \end{align}
%
    It can be shown that these equations can be obtained as saddle point equations from the so called Bethe free entropy
defined as 
    $\Phi_\text{Bethe} = \log Z^{\rm Bethe}(Y,T)/N$ where $Z^{\rm Bethe}$ is the Bethe approximation to the partition function which is defined as the normalization of the posterior measure. 
    The expression of the Bethe free
    entropy per variable can be computed in a standard way (see \cite{MM09}) and it is given by
\begin{equation}
    \Phi_\text{Bethe} = \frac{1}{N} \left( \sum_i\log Z_i + \sum_{i\le j}\log Z_{ij} +
    \sum_{i_1\le \dots \le i_p}\log Z_{i_1\dots i_p} -
    \sum_{i(ij)}\log Z_{i,ij} - \sum_{i(ii_2\dots i_p)}\log
    Z_{i(ii_2\dots i_p)} \right)\;,
\end{equation}
where
\begin{align*}
    & Z_i = \int dx_i P_X(x_i) \prod_j \tilde{m}_{ij\rightarrow i}(x_i) \prod_{(i_2\dots i_p)} \tilde{t}_{ii_2\dots i_p\rightarrow i}(x_i),
    \\
    & Z_{ij} = \int \prod_{j(\neq i)}\left[dx_{j}m_{j\rightarrow
      ij}(x_j)\right]   \prod_{i<
      j}e^{-\frac1{2\Delta_2}\left(Y_{ij}-\frac{x_ix_j}{\sqrt{N}}\right)^2}\, ,
    \\
    & Z_{i_1\dots i_p} = \int
      \prod_{l=1}^p\left[dx_{i_l}t_{i_l\rightarrow i_1\dots
      i_p}(x_{i_l})\right] \prod_{
      i_1<\dots<i_p}e^{-\frac1{2\Delta_p}\left(T_{i_1\dots
      i_p}-\frac{\sqrt{(p-1)!}}{N^{(p-1)/2}}x_{i_1}\dots
      x_{i_p}\right)^2}\, ,
    \\
    & Z_{i(ij)} = \int dx_im_{i\rightarrow ij}(x)\tilde{m}_{ij\rightarrow i}(x_i),
    \\
    & Z_{i(ii_2\dots i_p)} = \int dx_it_{i\rightarrow ii_2\dots i_p}(x)\tilde{t}_{ii_2\dots i_p\rightarrow i}(x_i)
\end{align*}
are a set of normalization factors. Using the Gaussian approximation for the messages and employing the same TAPyification procedure used to get the AMP equations
we obtain the Bethe free entropy density as
\begin{equation}\label{eq:free entropy Bethe}
    \begin{split}
        \Phi_\text{Bethe} &=\frac{1}{N}\sum_i \log
        {\cal Z}(A^{(p)}+A^{(2)},B^{(p)}_i+B^{(2)}_i)+\frac{p-1}p \frac{1}{N} \sum_i\Bigg[-B_i^{(p)}\hat{x}_i + A_i^{(p)}\frac{\hat{x}_i^2+\sigma_i}2\Bigg]+\\
        &+\frac{p-1}{2p\Delta_p}\left(\frac{\sum_i\hat{x}_i^2}N\right)^{p-1}\left(\frac{\sum_i\sigma_i}N\right)+\frac{1}{2N}\sum_i\Bigg[-B_i^{(2)}\hat{x}_i
        +
        A_i^{(2)}\frac{\hat{x}_i^2+\sigma_i}2\Bigg]+\frac{1}{4\Delta_2}\left(\frac{\sum_i\hat{x}_i^2}N\right)\left(\frac{\sum_i\sigma_i}N\right)\; ,
    \end{split}
\end{equation}
where we used the variables defined in eqs. (\ref{eq:AMP B2}-\ref{eq:AMP Ap}) for sake of compactness
and ${\cal Z}(A,B)$ is defined as
\begin{equation}
{\cal Z}(A,B)=\int dx P_X(x)e^{Bx-\frac{Ax^2}2} =
    \frac1{\sqrt{A+1}}e^{\frac{B^2}{2(A+1)}}\;.  \label{eq:ZAB}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Averaged free entropy and its proof}

Eq.~(\ref{eq:free entropy Bethe}) represents the Bethe free entropy for a single realization of the factor nodes in the large size limit. Here we wish to discuss the actual, exact, value of this free entropy, that is:
\[f_N(Y,T)=\frac {\log Z(Y,T)}N \]
This is a random variable, since it depends a priori on the planted signal and the noise in the tensor and matrices. However one expects that, since free entropy is an intensive quantity, we expect from the statistical physics intuition that  it should be self averaging and concentrate around its mean value in the large $N$ limit \cite{MPV87}. In fact, this is easily proven. First, since the spherical model has a rotational symmetry, one may assume the planted assignment could be any vector on the hyper-sphere, and we might as well suppose it is the uniform one $x_i^*=1 \forall ~i$: the true source of fluctuation comes from the noise $Y$ and $T$. These can be controlled by noticing that the free entropy is a Lipshitz function of the Gaussian random variable $Y$ and $T$. Indeed:
%
\[ \partial_{Y_{ij}} f_N(Y,T)=\frac 1{\Delta_2 N \sqrt{N}}\langle  x_i x_j \rangle \]
so that the free energy $f_N$ is Lipschitz with respect to $Y$ with constant 
\[L=\frac 1{\Delta_2 N \sqrt{N}} \sqrt{\sum_{i<j} \langle  x_i x_j \rangle^2 }\le  \frac 1{\Delta_2 N \sqrt{N}} \sqrt{\frac12 \sum_{i,j} \langle  x_i x_j \rangle^2 } 
= \frac 1{\Delta_2 N \sqrt{N}} \sqrt{\frac 12 \sum_{i,j} \langle  x_i \tilde x_i x_j \tilde x_j\rangle } \]
where  $\tilde x$ represent a copy (or replica) of the system. In this case 
\[L \le \frac 1{\Delta_2 N \sqrt{N}} \sqrt{N^2 \langle \left( \frac{\sum_i x_i \tilde x_i}{N}\right)^2\rangle }=
 \frac {\sqrt{\langle q^2\rangle}}{\Delta_2 \sqrt{N}} \]
where $q$ is the overlap between the two replica $x$ and $\tilde x$, that is bounded by one on the sphere, so $L \le \frac 1{\Delta_2 \sqrt{N}}$. Therefore, by Gaussian concentration of Lipschitz functions (the Tsirelson-Ibragimov-Sudakov inequality \cite{boucheron2004concentration}), we have for some constant $K$:
\begin{equation}
\textrm{Pr}\left[ | f_n-\mathbb{E}_Y f_n | \ge t \right]\le 2 e^{-N t^2/K}
\end{equation}
and it particular any fluctuation larger than $O(1/\sqrt{N})$ is (exponentially) rare. A similar computaton shows that $f_N$ also concentrates with respect to the tensor $T$. This shows that in the large size limit, we can consider the averaged free entropy:
\[ {\cal F}_N \equiv \frac{1}{N} \mathbb{E} \left[ \log Z_N
                \right] \]

With our (non-rigorous) statistical physics tools, this can be obtained by averaging Eq.~(\ref{eq:free entropy Bethe}) over the disorder, see for instance \cite{LKZ17}, and this yields an expression for the free energy called the replica symmetric (RS) formula:
%
\begin{equation}
\Phi_\text{RS}=\lim_{N \to \infty} \mathbb{E}_{Y,T} \frac {\log Z(Y,T)}N\,.
\label{RS_result}
\end{equation}
%
We now state precisely the form of $\Phi_{\rm RS}$ and prove the validity of Eq.~(\ref{RS_result}).
% 
The RS free entropy for any prior distribution $P_X$ reads as 
%
\begin{equation}\label{eq:free entropy generic}
	\begin{split}
    	\Phi_\text{RS}& \equiv {\rm max}_m \tilde\Phi_\text{RS}(m)  \quad
        {\rm where} \\
       \tilde\Phi_\text{RS}(m) &=\mathbb{E}_{W,x^*}\left[\log\left[{\cal Z}\left(\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p},\left(\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p}\right)x^*+\sqrt{\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p}}W\right)\right]\right]
    	-\frac1{4\Delta_2}m^2-\frac{p-1}{2p\Delta_p}m^p\;,
	\end{split}
\end{equation}
where $W$ is a Gaussian random variable of zero mean and unit variance
and $x^*$ is a random variables taken from the prior $P_X$.
We remind that the function ${\cal Z}(A,B)$ is defined via Eq.~(\ref{eq:ZAB}).
%

For Gaussian prior $P_X$, which is the one of interest here, we obtain
\begin{equation}
   \tilde\Phi_\text{RS}(m)=-\frac12\log\left(\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p}+1\right)+\frac12\left(\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p}\right)-\frac1{4\Delta_2}m^2-\frac{p-1}{2p\Delta_p}
   m^p\;.
    \label{eq:Phi_sph}
\end{equation}
%
The expression given in the main text is slightly different but can be
obtained as follow. First notice that the extremization condition for
$\tilde\Phi_\text{RS}(m)$ reads
%
\begin{equation}
        m= 1-\frac1{1+\frac{m}{\Delta_2}+\frac{m^{p-1}}{\Delta_p}}
        \label{eq:extrem}
\end{equation}
%
and by plugging this expression in Eq.~(\ref{eq:Phi_sph}) we recover the more compact expression
$\Phi_\text{RS}(m)$ showed in the main text: 
\begin{equation}
   \Phi_\text{RS}(m)=\frac12\log\left(1-m\right)+\frac{m}2+\frac{m^2}{4\Delta_2}+\frac{m^p}{2p\Delta_p}\;. 
\end{equation}
%
The two expressions $\Phi_\text{RS}(m)$ and $\tilde \Phi_\text{RS}(m)$
are thus equal for each value of $m$ that satisfy Eq.~(\ref{eq:extrem}). 
The parameter $m$ can be interpreted as the average correlation between the true and the estimated signal
\begin{equation}
m=\frac{1}{N} \sum_{i=1}^N x_i^*\hat x_i\:.
\end{equation}
The average minimal mean squared error (MMSE) can be obtained from the maximizer $m$ of the average Bethe free entropy as
\begin{equation}
   {\rm MMSE}\equiv \frac{1}{N}\sum_{i=1}^N \overline{(x_i^*-\hat x_i)^2} = 1 - m^*\, , \quad {\rm where} \quad    m^* = {\rm
     argmax} \tilde\Phi_\text{RS}(m) \, . 
\label{V-MMSE}
\end{equation}
where the overbar stands for the average over the signal $x^*$ and the noise of the two Gaussian channels.

The validity of Eq.~(\ref{eq:free entropy generic}) can be
proven rigorously for every prior having a bounded second moment. The
proof we shall present is a straightforward generalization of the one
presented in \cite{MiolaneTensor} for the pure tensor case, and in
\cite{MiolaneXX} for the matrix case, and it is based on two main
ingredients. The first one is the Guerra interpolation method applied on the Nishimori line
\cite{korada2009exact,krzakala2016mutual,MiolaneXX}, in which we
construct an interpolating Hamiltonian that depends on a parameter $t\in[0;1]$ that is
used to move from the original Hamiltonian of Eq.~(\ref{eq:Hamiltonian}), to the one
corresponding to a scalar denoising problem whose free entropy is
given by the first term in Eq.~(\ref{eq:free entropy generic}).  The second ingredient is 
the Aizenman-Sims-Starr method \cite{aizenman2003extended} which is
the mathematical version of the cavity method (note that other
techniques could also be employed to obtain the same results, see
\cite{XXT,barbier_stoInt,AlaouiKrzakala,mourrat2018hamilton}). The theorem we want to prove is:

\begin{theorem}[Replica-Symmetric formula for the free energy]\label{thm1}
	Let $P_X$ be a probability distribution over \,$\R$, with
        finite second moment $\Sigma_X$. Then, for all $\Delta_2>0$ and $\Delta_p>0$
	\begin{equation} \label{eq:lim_F}
		{\cal F}_N \equiv \frac{1}{N} \mathbb{E} \left[ \log Z_N
                \right] \xrightarrow[N \to \infty]{} \sup_{m \geq 0}
              \tilde  \Phi_{\rm RS}(m) \equiv \Phi_\text{\rm RS}(\Delta_2,\Delta_p)\,.
	\end{equation}
        For almost every $\Delta_2>0$ and $\Delta_p>0$, $\tilde \Phi_{\rm RS}$
        admits a unique maximizer $m$ over $\R_+ \times \R_+$ and
	$$
	{\rm T-MMSE}_N \xrightarrow[N \to \infty]{} 
	\Sigma_X^p - (m^*)^p \, ,
	$$
	$$
	{\rm M-MMSE}_N \xrightarrow[N \to \infty]{} 
	\Sigma_X^2 - (m^*)^2 \,.
	$$
\end{theorem}
%
Here, we have defined the tensor-MMSE  $\text{T-MMSE}_N$ by the error in
reconstructing the tensor:
\begin{align*}
	\text{T-MMSE}_N(\Delta_2,\Delta_p)=
	\inf_{\hat{\theta}} \left\{ 
		\frac{p!}{N^p} \sum_{i_1 < \dots < i_p} \left(
			x^0_{i_1} \dots x^0_{i_p}
			- \hat{\theta}(Y)_{i_1 \dots i_p} 
		\right)^2
	\right\} \,,
\end{align*}
and the  matrix-MMSE  $\text{M-MMSE}_N$ by the error in
reconstructing the matrix:
\begin{align*}
	\text{M-MMSE}_N(\Delta_2,\Delta_p)=
	\inf_{\hat{\theta}} \left\{ 
		\frac{2}{N^2} \sum_{i < j} \left(
			x^0_{i} x^0_{j}
			- \hat{\theta}(Y)_{i,j} 
		\right)^2
	\right\} \,,
\end{align*}
where in both cases the infimum is taken over all measurable functions
$\hat{\theta}$ of the observations $Y$.

The result concerning the MMSE is a simple application of the I-MMSE
theorem \cite{GuoShamaiVerdu_IMMSE}, that relates the derivative of the
free energy with respect to the noise variances and the MMSE. 
The details of the arguments are the same than in
the matrix ($p=2$) case (\cite{MiolaneXX}, corollary 17) and the tensor
one (\cite{MiolaneTensor}, theorem 2). Indeed, as discussed  in \cite{MiolaneXX, MiolaneTensor},
 these M-MMSE and T-MMSE results implies the vector MMSE
result of Eq.~(\ref{V-MMSE}) when $p$ is odd, and thus in particular for the
$p=3$ case discussed in the main text.
 


\paragraph{Sketch of proof}
%
In this section we give a detailed sketch of the proof theorem
$1$. Following the techniques used in many recent works
\cite{korada2009exact,krzakala2016mutual,
  XXT,MiolaneXX,MiolaneTensor,barbier_stoInt,AlaouiKrzakala,barbier2017phase}, we shall
make few technical remarks:
\begin{itemize}
\item We will consider only priors with bounded
  support, $\text{supp}(P_X) = S \subset [-K;K]$. This allows to switch
  integrals and derivatives without worries. This condition can then
  be relaxed to unbounded distributions with bounded second moment
  using the same techniques as the ones that we are going to present, and
  the proof is therefore valid in this case. This is detailed for
  instance in \cite{MiolaneXX} sec. 6.2.2.
\item Another key ingredient is the introduction of a
  small perturbation in the model that takes the form of a small
  amount of side information.  This kind of techniques are frequently
  used in statistical physics, where a small ``magnetic field''
  forces the Gibbs measure to be in a single pure state
  \cite{georgii2011gibbs}. It has also been used in the context
  of coding theory \cite{Macris2007} for the same reason.
  In the context of Bayesian inference, we follow the generic scheme
  proposed by Montanari in \cite{andrea2008estimating} (see also
  \cite{coja2017information}) and add a small additional source of
  information that allows the system to be in a single pure state so that
  the overlap concentrates on a single value.  This source depends on
  Bernoulli random variables
  $L_i\stackrel{\text{i.i.d.}}{\sim}\text{Bern}(\epsilon)$, $i\in[N]$;
  if $L_i=1$, the channel, call it $A$, transmits the correct
  information. We can then consider the posterior of this new problem,
  $P(X|A,Y,T)$, and focus on the associated free energy density
  $F_{N,\epsilon}$ defined as the expected value of the average of the
  logarithm of normalization constant divided by the number of
  spins. Then we can immediately prove that for all $N\ge1$ and
  $\epsilon,\epsilon'\in[0;1]$ it follows:
  $\left|F_{N,\epsilon}-F_{N,\epsilon'}\right|\leq
  \left(\frac{K^{2p}}{\Delta_p}+\frac{K^4}{\Delta_2}\right)|\epsilon-\epsilon'|$. This
  allows (see for instance \cite{MiolaneTensor}) to obtain the
  concentration of the posterior distribution around the replica
  parameter ($q=\frac1N\langle x^{(1)}\cdot x^{(2)}\rangle$)
\begin{align}
	& \mathbb{E} \left\langle\left(\frac{x^{(1)}\cdot x^{(2)}}N - q\right)^2\right\rangle \stackrel{N\rightarrow\infty}{\longrightarrow0} \;; \\
	& \mathbb{E} \left\langle\left(\frac{x^*\cdot x}N -
          q\right)^2\right\rangle
          \stackrel{N\rightarrow\infty}{\longrightarrow0} \;, 
\end{align}
where $x,x^{(1)},x^{(2)}$ are sampled from the posterior distribution
and the averages $\langle\cdot\rangle$ and $\mathbb{E}[\cdot]$ are
respectively the average over the posterior measure and the
remaining random variables.
\item Finally, a fundamental property of inference problems which is a direct
  consequence of the Bayes theorem\footnote{And the fact that we are in the Bayes optimal setting where we know the statistical properties of the signal, namely the prior, and the statistical properties of the channels, namely $\Delta_2$ and $\Delta_p$.}, is
  the so-called Nishimori symmetry \cite{nishimori2001statistical,REVIEWFLOANDLENKA}: Let $(X,Y)$ be a couple of random variables
  on a polish space. Let $k \geq 1$ and let $X^{(1)}, \dots, X^{(k)}$
  be $k$ i.i.d.\ samples (given $Y$) from the distribution
  $P(X=\cdot \, | \, Y)$, independently of every other random
  variables. Let us denote $\langle \cdot \rangle$ the expectation
  with respect to $P(X=\cdot \, | \, Y)$ and $\mathbb{E}$ the
  expectation with respect to $(X,Y)$. Then, for all continuous
  bounded function $f$
	$$
	\mathbb{E} \langle f(Y,X^{(1)}, \dots, X^{(k)}) \rangle
	=
	\mathbb{E} \langle f(Y,X^{(1)}, \dots, X^{(k-1)}, X) \rangle \,.
	$$
        While the consequences of this identity are important, the proof is rather simple: It
        is equivalent to sample the couple $(X,Y)$ according to its
        joint distribution or to sample first $Y$ according to its
        marginal distribution and then to sample $X$ conditionally to
        $Y$ from its conditional distribution $P(X=\cdot \, | \,
        Y)$. Thus the $(k+1)$-tuple $(Y,X^{(1)}, \dots,X^{(k)})$ is
        equal in law to $(Y,X^{(1)},\dots,X^{(k-1)},X)$.
\end{itemize}
The proof of Theorem \ref{thm1} is obtained by using the Guerra interpolation technique to prove a lower bound for the free entropy and
then by applying the Aizenman-Sims-Star scheme to get a matching upper bound.


\paragraph{Lower bound: Guerra interpolation} We now move to the core
of the proof. The first part combines the Guerra interpolation method
\cite{guerra2002thermodynamic} developed for matrices in
\cite{krzakala2016mutual} and tensors in \cite{MiolaneTensor}. 

Consider the interpolating Hamiltonian depending of $t\in[0,1]$
\begin{equation}\label{eq:interpolating Hamiltonian}
	\begin{split}
		\mathcal{H}_{N,t} &= - \sum_{i<j}\left[\frac{\sqrt{t}}{\Delta_2\sqrt{N}}Y_{ij}x_ix_j +\frac{t}{2\Delta_2N}(x_ix_j)^2\right] +\\
		& - \sum_{i_1<\dots<i_p}\left[\frac{\sqrt{t(p-1)!}}{\Delta_pN^{\frac{p-1}2}}T_{i_1\dots i_p}x_{i_1}\dots x_{i_p} + \frac{t(p-1)!}{2\Delta_pN^{p-1}}(x_{i_1}\dots x_{i_p})^2\right] + \\
		& - \sum_j\left[\sqrt{1-t}\sqrt{\frac{m^{p-1}}{\Delta_p}+\frac{m}{\Delta_2}}W_jx_j+(1-t)\left(\frac{m^{p-1}}{\Delta_p}+\frac{m}{\Delta_2}\right)x_j^*x_j+\frac{1-t}2\left(\frac{m^{p-1}}{\Delta_p}+\frac{m}{\Delta_2}\right)x_j^2\right]\,,
	\end{split}
\end{equation}
%
where we have for $t=1$ the regular Hamiltonian and for $t=0$
the first term of Eq.~(\ref{eq:free entropy generic}) where $W_j$ are
i.i.d. canonical Gaussian variables.  More importantly, for all
$t\in[0,1]$ we can show that the Hamiltonian above can be seen as the one emerging for an appropriate inference problem, so that
the Nishimori property is kept valid  for generic $t\in [0,1]$ \cite{krzakala2016mutual}.

Given the interpolating Hamiltonian we can write the corresponding
Gibbs measure,
\begin{equation}
P(x|W,Y,T) = \frac1{\mathcal{Z}_{N,t}}P_X(x)e^{H_{N,t}(x)}\, ,
\end{equation}
and the interpolating free entropy
\begin{equation}
\psi_N(t) \doteq
\frac1N\mathbb{E}\left[\log\mathcal{Z}_{N,t}\right]\, ,
\end{equation}
whose boundaries are $\psi_N(1) = \frac1N\mathcal{F}_N$ (our target) and
$\psi_N(0) = \frac1N\tilde\Phi_\text{RS} + \frac1{4\Delta_2}m^2 +
\frac{p-1}{2p\Delta_p}m^p$.
We then use the fundamental theorem of calculus to write
\begin{equation}
	\mathcal{F}_N = \psi_N(1) = \psi_N(0) +\frac1N\underbrace{\mathbb{E}\int_0^1\left(-\frac{\partial\log\mathcal{Z}_{N,t}}{\partial t}\right)dt}_{\doteq \mathcal R}\,.
\end{equation}
We work with the second term and use Stein's lemma which, given a
well behaving function $g$, provides the useful relation for a
canonical Gaussian variable $Z$: $\mathbb{E}_Z[Zg(Z)] =
\mathbb{E}_Z[g'(Z)]$. This yields
\begin{equation*}
	\begin{split}
		\mathcal{R} & = -\mathbb{E}\int_0^1\left[\frac1{\mathcal{Z}_{N,t}}\int dx^N \frac{\partial \mathcal{H}_{N,t}(x)}{\partial t}P_X(x)e^{\mathcal{H}_{N,t}(x)} \right]dt = -\mathbb{E}\int_0^1\left\langle \frac{\partial \mathcal{H}_{N,t}(x)}{\partial t} \right\rangle dt \\
		& = -\mathbb{E}\int_0^1\left\langle \sum_{i<j}\frac1{\Delta_2N}(x_i^*x_ix_j^*x_j) + \sum_{i_1<\dots<i_p}\frac{(p-1)!}{\Delta_2N^{p-1}}(x_{i_1}^*x_{i_1}\dots x_{i_p}^*x_{i_p}) - \sum_i\left(\frac{m}{2\Delta_2}+\frac{m^{p-1}}{2\Delta_p}\right)x_i^*x_i \right\rangle dt \\
		& =
                \mathbb{E}\int_0^1\left[\frac1{4\Delta_2}\left\langle
                    \left(\frac{x\cdot x^*}N\right)^2 - 2
                    m\left(\frac{x\cdot x^*}N\right)\right\rangle +
                  \frac1{2p\Delta_p}\left\langle \left(\frac{x\cdot
                        x^*}N\right)^p - p m^{p-1}\left(\frac{x\cdot
                        x^*}N\right)\right\rangle\right] dt\,. 
	\end{split}
\end{equation*}
where we have used the Nishimori property to replace terms such as
$\langle x\rangle^2$ by $\langle x x^* \rangle$. At this point, we can
write
\begin{eqnarray}
		\mathcal{R}&=&
                \mathbb{E}\int_0^1\left[\frac1{4\Delta_2}\left\langle
                    \left(\frac{x\cdot x^*}N\right)^2 - 2
                    m\left(\frac{x\cdot x^*}N\right)\right\rangle \right]dt
                  +\mathbb{E}\int_0^1\left[
                  \frac1{2p\Delta_p}\left\langle \left(\frac{x\cdot
                        x^*}N\right)^p - p m^{p-1}\left(\frac{x\cdot
                        x^*}N\right)\right\rangle\right]
                               dt\, \nonumber  \\
                &=&-\frac {m^2}{4\Delta_2} + \frac {1}{4\Delta_2} 
                \mathbb{E}\int_0^1\frac1{4\Delta_2}\left\langle
                    \left(\frac{x\cdot x^*}N-m\right)^2 \right\rangle dt
                 + \frac1{2p\Delta_p}\mathbb{E}\int_0^1\
                 \left\langle \left(\frac{x\cdot
                        x^*}N\right)^p - p m^{p-1}\left(\frac{x\cdot
                        x^*}N\right)\right\rangle
                    dt\,. \nonumber \\
\end{eqnarray}
The first integral is clearly positive. The second one,
however, seems harder to estimate. We may, however, use a simple
convexity argument on the function $f(x) = x^k$. Indeed observe that
$\forall\;a,b\ge0$ and $p\ge1$: $a^p-p b^{p-1}a \ge (1-p)b^p$. We would like
to use this property but there is the subtlety that we need $x\cdot x^*$ to be
non-negative. To bypass this problem we can add again a small
perturbation that forces $x \cdot x^*$ to concentrate around a
non-negative value, without affecting the ``interpolating free
entropy'' $\psi_N(t)$ in the $N \to \infty$ limit. This is, again, the
argument used in \cite{MiolaneTensor} and originally in
\cite{korada2009exact}. In this way we can write
\begin{eqnarray}
		\mathcal{R} &\ge& -\frac {m^2}{4\Delta_2}+ \mathbb{E}\int_0^1\left[\frac1{4\Delta_2}\left\langle
                    \left(\frac{x\cdot x^*}N\right)^2 - 2
                    m\left(\frac{x\cdot x^*}N\right)\right\rangle \right]dt + 
\frac{(1-p)m^p}{4\Delta_2}         \, \nonumber
  \\
 &\ge& -\frac {m^2}{4\Delta_2} - \frac{(p-1)m^p}{4\Delta_2}       \:.       
\end{eqnarray}
This concludes the proof and yields the lower bound:
\begin{equation}
	\mathcal{F}_N \ge \psi_N(0) - \frac1{4\Delta_2}m^2 -
        \frac{p-1}{2p\Delta_p}m^p   =
        \frac1N\tilde\Phi_\text{RS}(m)   \, ,
\end{equation}
so that for all $m\ge 0$
\begin{align*}
  \liminf_{N \to \infty} {\cal F}_N = \liminf_{N \to \infty}
  \psi_N(1) &= \liminf_{N \to \infty} \left[\psi_N(0) +
              \int_0^1 \psi'_N(t) dt \right]  \geq \tilde \Phi_{\rm RS}(m) \,.
\end{align*}
        
\paragraph{Upper bound: Aizenman-Sims-Starr scheme.} The matching
upper bound is obtained using the Aizenman-Sims-Starr
scheme \cite{aizenman2003extended} . This is a particularly effective
tool that has been already used for these problems, see for example
\cite{MiolaneXX,coja2017information,MiolaneTensor}. The method goes as follows. Consider the
original system with $N$ variables, $\mathcal{H}_N$ and add an new variable
$x_0$ so that we get an Hamiltonian $\mathcal{H}_{N+1}$. 
Define the Gibbs measures of the two systems, the first with $N$ variables and the second with $N+1$ variables, and consider the two relative free entropies.
 Call
$A_N = \mathbb{E}\left[\log\mathcal{Z}_{N+1}\right] -
\mathbb{E}\left[\log\mathcal{Z}_{N}\right]$ their difference.  First, we notice that we
have $\lim\sup_N\mathcal{F}_N \le \lim\sup_NA_N$ because 
$$
{\cal  F}_N=\mathbb{E} \frac 1N \log {Z_N} = \frac 1N \mathbb{E} \log  \left(\frac{Z_N}{Z_{N-1}} \frac{Z_{N-1}}{Z_{N-2}} \ldots\frac{Z_1}{Z_0} \right)= \frac 1N \sum_i A_i \le \sup_i A_i\, .
$$
 Moreover, we can separate the contribution of the additional variable in the Hamiltonian ${\cal H}_{N+1}$ so that
$\mathcal{H}_{N+1} = \tilde{\mathcal{H}}_N + x_0 z(x) + x_0^2 s(x)$,
with $x = (x_1,\dots,x_N)$, and
\begin{align*}
	& z(x) = \frac1{\sqrt{\Delta_2(N+1)}}\sum_{i=1}^N Z_{0i}x_i + \frac{\sqrt{(p-1)!}}{\sqrt{\Delta_p}(N+1)^{(p-1)/2}}\sum_{1\le i_1<\dots<i_{p-1}\le N}Z_{0i_1\dots i_{p-1}}x_{i_1}\dots x_{i_{p-1}} + \\
	&\quad + \frac1{\Delta_2(N+1)}\sum_{i=1}^N x_0^*x_i^*x_i +\frac{(p-1)!}{\Delta_p(N+1)^{p-1}}\sum_{1\le i_1<\dots<i_{p-1}\le N} x_0^*x_{i_1}^*x_{i_1}\dots x_{i_{p-1}}^*x_{i_{p-1}}
	\\
	& s(x) = - \frac1{2\Delta_2(N+1)}\sum_{i=1}^N x_i^2 - \frac{(p-1)!}{2\Delta_p(N+1)^{p-1}}\sum_{1\le i_1<\dots<i_{p-1}\le N}(x_{i_1}\dots x_{i_{p-1}})^2
\end{align*}
and $\mathcal{H}_{N+1}$ is the same expression as Eq.~(\ref{eq:Hamiltonian}) where the $N$ in the denominators are replaced by $N+1$. We rewrite also $\mathcal{H}_N(x)$ as a perturbation of $\tilde{\mathcal{H}}_N$: $\mathcal{H}_N(x) = \tilde{\mathcal{H}}_N(x) + y(x) + O(1)$ with

\begin{align*}
	& y(x) = \frac1{\sqrt{\Delta_2N}}\sum_{i<j}V_{ij}x_ix_j + \sqrt{p-1}\frac{\sqrt{(p-1)!}}{\sqrt{\Delta_p}N^{p/2}}\sum_{i_1<\dots<i_p}V_{i_1\dots i_p}x_{i_1}\dots x_{i_p} + \\
	&\quad + \frac1{N^2}\sum_{i<j}\left[x_i^*x_ix_j^*x_j-\frac12(x_ix_j)^2\right] +(p-1)!\frac{p-1}{N^p}\sum_{i_1<\dots<i_p}\left[x_{i_1}^*x_{i_1}\dots x_{i_p}^*x_{i_p}-\frac12(x_{i_1}\dots x_{i_p})^2\right],
\end{align*}
where the $Z$s and the $V$s are standard Gaussian random variables.

Finally we can observe the partition functions $Z_N$ can be interpreted
as ensemble averages with respect to $\tilde{\mathcal{H}}_N$. Thus
$A_N = \mathbb{E}\log\left\langle\int P_X(x_0)e^{x_0 z(x)+x_0^2
    s(x)}dx_0 \right\rangle_{\tilde{\mathcal{H}}_N} -
\mathbb{E}\log\left\langle
  e^{y(x)}\right\rangle_{\tilde{\mathcal{H}}_N}$. Now, using the
Nishimori property and the concentration of the overlap around a
non-negative value ---that we denote $m(Y,T)$ since it depends explicitly on the disorder--- it yields (see \cite{MiolaneXX}, see section 4.3 for
details) \eqref{eq:free entropy generic} in the thermodynamic limit, with $m(Y,T)$ instead of $m$. From this, we can now obtain the upper bound that concludes the proof:
\begin{equation}
	\limsup_N \mathcal{F}_N \le \limsup_N A_N \le \limsup_N \mathbb{E}_{Y,T}\tilde\Phi_\text{RS}[m(Y,T)] \le  \limsup_N \sup_{{m}}\Phi_\text{RS}({m}) \le \tilde\Phi_\text{RS}\,.
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{State evolution of AMP and its analysis}\label{subsec:SE}

\begin{figure}[h]
    \centering
    \includegraphics[scale=.5]{img/PhaseDiagram_2+3_AMP.pdf}
    \includegraphics[scale=.5]{img/PhaseDiagram_2+4_AMP.pdf}
    \caption{\emph{On the left}: Phase diagram of the spiked matrix-tensor model for
      $p=3$. The phase diagram identifies four regions: easy (green),
      impossible (red), and hard (orange). The lines correspond to 
      different phase transitions namely the stability threshold (dashed black),
      the information theoretic threshold (solid red), the algorithmic
      threshold (solid cyan), and the dynamical threshold (dotted
      orange). The vertical cuts represent the section along which the magnetization is plotted in Fig.~\ref{fig:phase diagram p=3 sections}.
      \emph{On the right}: Phase diagram of the spiked matrix-tensor model for
      $p=4$. The main difference with respect to case $p=3$,
       is that the algorithmic
      spinodal (solid cyan) is strictly above the stability threshold
      (dashed black). The hybrid-hard phase appears between these two
      lines (combined green and orange color). The vertical cuts represent the section along which the magnetization is plotted in Fig.~\ref{fig:phase diagram p=4 sections}.
}
    \label{fig:phase diagram p=3}
\end{figure}


The dynamical evolution of the AMP algorithm in the large $N$ limit is described by the so-called State Evolution (SE) equations. 
The derivation of these equations can be straightforwardly done using the same techniques developed in \cite{LKZ17}.
They can be written in terms of two dynamical order parameters namely $m^t = \sum_i
\hat{x}_i^tx_i^*/N$, which encodes for the alignment of the current estimation $\hat x_i^t$ of the components of the signal with the signal itself at
time $t$ and $q^t = \sum_i \hat{x}_i^t\hat{x}_i^t/N$. 
Finally, using the Nishimori symmetry it can be shown that $m^t = q^t$ at all times\footnote{Note that AMP satisfies the Nishimori property at all times while this condition is violated on the run by the Langevin dynamics. In that case the Nishimori symmetry is recovered only when equilibrium is reached and therefore it is violated when the Langevin algorithm gets trapped in the glass phase, see below.}, see e.g. \cite{REVIEWFLOANDLENKA}, and therefore the evolution
of the algorithm is characterized by a single order parameter
$m^t$ whose dynamical evolution is given by 
\begin{equation}
        m^{t+1}= 
1-\frac1{1+\frac{m^t}{\Delta_2}+\frac{(m^t)^{p-1}}{\Delta_p}}\;\;.
        \label{eq:AMP SE}
\end{equation}
If we initialize the configuration of the estimator $\hat x$ at random, the initial value of $m$ will be equal to zero on average.
However finite size fluctuations will produce by chance a small bias towards the signal and therefore it is more meaningful 
to consider the initialization to be $m^{t=0}=\epsilon$
being $\epsilon$ an arbitrarily small positive number.
We will call $m_{\rm AMP}$ the fixed point of Eq.~(\ref{eq:AMP SE}) reached
from this infinitesimal initialization. 
The
mean-square-error (MSE) reached by AMP after convergence is then given by ${\rm MSE}_{\rm AMP} = 1-m_{\rm
  AMP}$.

We underline that Eq.~(\ref{eq:AMP SE})  can be proven 
rigorously following \cite{javanmard2013state,richard2014statistical}.
Finally we note that the fixed point of the SE satisfies the very same Eq.~(\ref{eq:extrem}) that 
gives the replica
free entropy.
In the rest of this section we will study the fixed points of Eq.~(\ref{eq:AMP SE}). This will allow too determine the phase diagram of the spiked
matrix-tensor model. 

We start by observing that $m=0$ is a fixed point of Eq.~(\ref{eq:AMP SE}). 
However in order to understand wether it is a possible attractor of the AMP dynamics
we need to understand its local stability. This can be obtained perturbatively by
expanding Eq.~(\ref{eq:AMP SE}) around $m=0$
\begin{equation}
		    m^{t+1}
    	=\frac{m^t}{\Delta_2}+\left(\frac{m^t}{\Delta_2}\right)^2-\frac{(m^t)^{p-1}}{\Delta_p}+O\left((m^t)^3\right)\;.
\end{equation}
It is clear that the non-informative fixed point $m=0$ is stable as long as
$\Delta_2>1$. We will call $\Delta_2=1$ the \emph{stability threshold}. 


\begin{figure}
    \centering
    \includegraphics[scale=.5]{img/PhaseDiagram_2+5.pdf}
     \includegraphics[scale=.5]{img/PhaseDiagram_2+10.pdf}

    \caption{\emph{On the left}: Phase diagram of the spiked matrix-tensor model for
      $p=5$. 
      \emph{On the right}: Phase diagram of the spiked matrix-tensor model for
      $p=10$.  
      In both cases we observe qualitatively the same scenario found in the right panel of Fig.~\ref{fig:phase diagram p=3}.
      }
    \label{fig:phase diagram p=5}
\end{figure}

When $p=3$ the SE equations are particularly simple
and the fixed points are written explicitly as 
\begin{equation}
    m_0=0\,;\quad \quad 
    m_\pm=\frac12\left[1-\frac{\Delta_3}{\Delta_2} \pm
           \sqrt{\left(1+\frac{\Delta_3}{\Delta_2}\right)^2-4\Delta_3}\right]\;.
\end{equation}
In the regime where $\Delta_2>1$, $m_0$ and $m_+$ are stable while
$m_-$ in unstable. When $\Delta_2$ becomes smaller than one, $m_+$
becomes the only non-negative stable solution and therefore $\Delta_2=1$ is also known as the \emph{algorithmic spinodal} since it corresponds to the point
where the AMP algorithm converges to the informative fixed point. 
The informative solution $m_+$ exists as long as $\Delta_2  \le   \Delta^{\rm dyn}_2 $, where we have defined the
 \emph{dynamical spinodal} by 
\begin{equation}
         \Delta^{\rm dyn}_2  = \frac{\Delta_3}{2 \sqrt{\Delta_3} -1} \, . 
\end{equation}


For a generic $p$ we cannot determine the values of the informative
fixed points explicitly but we can easily study Eq.~(\ref{eq:AMP SE}) numerically to get the full phase diagram.

Furthermore we can obtain the spinodal transition lines as follows. 
The key
observation is that the two spinodals are critical points of the
equation $\Delta_p(m;\Delta_2)$ where $\Delta_2$ is fixed, or
analogously $\Delta_2(m;\Delta_p)$ where $\Delta_p$ is fixed (to have
a pictorial representation of the idea you can see Fig. \ref{fig:phase
  diagram p=4 sections}). We call $x = m/\Delta_2 + m^{p-1}/\Delta_p$,
and $f_\text{SE}(x)\equiv 1 - \frac1{1+x}$, then
\begin{equation}
    \Delta_p\equiv\Delta_p(x;\Delta_2)=\frac{\left(f_\text{SE}(x)\right)^{p-1}}{x-\frac{f_\text{SE}(x)}{\Delta_2}}\;.
\end{equation}
%
Then the stationary points are implicitly defined by 
\begin{equation*}
    0=\frac{d\log\Delta_p}{d m}=\frac{\partial\log\Delta_p}{\partial x}(1+x)^2\propto (p-1)\frac{f_\text{SE}'(x)}{f_\text{SE}(x)}-\frac{1-\frac{f_\text{SE}'(x)}{\Delta_2}}{x-\frac{f_\text{SE}'(x)}{\Delta_2}}=\frac{\frac{2-p}{\Delta_2}+(1+x)(p-x-2)}{x(1+x)\left[x+1-\frac1{\Delta_p}\right]}\;,
\end{equation*}
giving
\begin{equation}\label{eq:spinodals x}
    x_\pm(\Delta_2)=\frac12\left[p-3\pm\sqrt{(p-1)^2-\frac4{\Delta_2}(p-2)}\right]\;.
\end{equation}
%
Finally $\Delta_p\left(x_\pm(\Delta_2);\Delta_2\right)$ describes the
two spinodals.  
%Observe that in the case $p=3$ one of the two spinodals just derived
%is unphysical.
We can also derive the tri-critical point, when the two spinodals meet, which is given by the zero discriminant condition on \eqref{eq:spinodals x}
\begin{equation}
    \left(\Delta_p^{\rm tri};1/\Delta_2^{\rm tri}\right)=\left(\frac{4(p-2)\left(\frac{p-3}{p-1}\right)^{p-1}}{(p-3)^2};\frac{(p-1)^2}{4(p-2)}\right)\;.
\end{equation}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Phase diagrams of spiked matrix-tensor model}

In this section we present the phase diagrams for the spiked
matrix-tensor model as a function of the two noise levels $\Delta_2$ and $\Delta_p$ and for several
values of $p$.  
These phase diagrams are plotted in Figs.~\ref{fig:phase diagram p=3} and \ref{fig:phase diagram p=5}.






\noindent Generically we can have four regions: 
\begin{itemize}
   \item {\bf Easy phase} (green), where the MSE obtained through AMP coincides with the MMSE which is better than random sampling of the prior. 
   \item {\bf Impossible phase} (red), where the MMSE and MSE of AMP coincide and are equal to 1 (meaning that $m^*=m_{AMP}$=0). 
   \item {\bf Hard phase} (orange),  where the MMSE is smaller than the MSE obtained from AMP and $m^*>m_{\rm AMP} \ge 0$.
   \item {\bf Hybrid-hard phase} \cite{Typology18} (mix of green and orange),
     is a part of the hard phase where the AMP
     performance is strictly better than random sampling from the prior,
     but still the MSE obtained this way does not match the MMSE, i.e. $m^*>m_{\rm AMP} > 0$.  The hybrid-hard phase can be found
      for $p \ge 4$.
\end{itemize}


\noindent All these phases are separated by the following transition lines:
\begin{itemize}
          \item The {\bf stability threshold} (dashed black line) at $\Delta_2=1$ for all $p$. This corresponds to the point where the uninformative fixed
            point $m=0$ looses its local stability. 
	\item The {\bf information theoretic
          threshold} (solid red line).  Here $m^*>0$ and the MMSE jumps to a value strictly smaller than one.
        \item The {\bf algorithmic threshold} (solid cyan line). This is
          where the fixed point of AMP jumps to the MMSE$<1$.
          For $p=3$ this line coincides with a segment
          of the stability threshold while for $p\ge 4$ it is
          strictly above.
	\item The {\bf dynamic
          threshold} (dotted orange line). Here the most informative fixed point (the one with largest $m_{\rm AMP}$) disappears.
\end{itemize}


In Figs.~\ref{fig:phase diagram p=3 sections}, and \ref{fig:phase diagram p=4 sections} we plot the 
evolution of the magnetization $m$, as found through the fixed points of the SE equation, for several fixed values of $\Delta_p$ and $p=3$ and $p=4$,
respectively. The values of $\Delta_p$ are identified by the vertical cuts in the phase diagrams of Fig.~\ref{fig:phase diagram p=3}.   

\begin{figure}[H]
    \centering
    \subfigure[Section S1: $p=3$, $\Delta_p=0.2$]{
        \includegraphics[scale=0.4]{img/{section_p3_Deltap0.200}.pdf}
    }
    \subfigure[Section S2:$p=3$, $\Delta_p=0.24$]{
        \includegraphics[scale=0.4]{img/{section_p3_Deltap0.240}.pdf}
    }
    \\
    \subfigure[Section S3: $p=3$, $\Delta_p=0.4$]{
        \includegraphics[scale=0.4]{img/{section_p3_Deltap0.400}.pdf}
    }
    \subfigure[Section S4: $p=3$, $\Delta_p=1.1$]{
        \includegraphics[scale=0.4]{img/{section_p3_Deltap1.100}.pdf}
    }
    \caption{Fixed points of Eq.~(\ref{eq:AMP SE}) as
      a function of $\Delta_2$
      for $p=3$ and several fixed values of $\Delta_p$. 
      The values of $\Delta_p$ correspond to the vertical cuts in the left panel of Fig.~\ref{fig:phase diagram p=3}. Solid
      lines are stable fixed point, dashed lines are unstable fixed
      points.  The blue line represent informative fixed points with positive
overlap with the signal while the orange line represent a uninformative fixed points
with no overlap with the signal. 
Starting from high $\Delta_2$ an informative fixed point appears at
the dynamical threshold (vertical dashed line) but is energetically
disfavored until the information theoretic threshold (vertical dotted
line) and finally it becomes the only stable solution crossing the
algorithmic threshold (vertical dotted-dashed line). When the
transition is continuous the three vertical threshold lines merge and
we have a single second order phase transition, which here occurs at
$\Delta_p \ge 1$.}
    \label{fig:phase diagram p=3 sections}
\end{figure}

\begin{figure}[H]
    \centering
    \subfigure[Section S1: $p=4$, $\Delta_p=0.1$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.100}.pdf}
    }
    \subfigure[Section S2: $p=4$, $\Delta_p=0.14$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.140}.pdf}
    }
    \centering
    \subfigure[Section S3: $p=4$, $\Delta_p=0.18$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.180}.pdf}
    }
    \subfigure[Section S4: $p=4$, $\Delta_p=0.24$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.240}.pdf}
    }
    \centering
    \subfigure[Section S5: $p=4$, $\Delta_p=0.27$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.270}.pdf}
    }
    \subfigure[Section S6: $p=4$, $\Delta_p=0.3$]{
        \includegraphics[scale=0.4]{img/{section_p4_Deltap0.300}.pdf}
    }
    \caption{Fixed points Eq.~(\ref{eq:AMP SE}) as
      a function of $\Delta_2$
      for $p=4$ and several fixed values of $\Delta_p$. The values of $\Delta_p$ correspond to the vertical cuts of the right panel of Fig.~\ref{fig:phase diagram p=3}.
       The situation is qualitatively similar to Fig.~\ref{fig:phase diagram p=3 sections}, the difference being only the presence of the hybrid-hard phase. 
       We can observe that when the transition is discontinuous, figure from (a) to (e), for $1/\Delta_2>1.0$ the uninformative solution becomes unstable and continuously goes to a stable-informative solution which is not the optimal one.} 
    \label{fig:phase diagram p=4 sections}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Langevin Algorithm and its state evolution}\label{sec:dynamics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The main goal of our analysis is to compare AMP with the performance of the Langevin dynamics. The advantage of the spiked matrix-tensor model is that in this case the Langevin dynamics can be studied in the large $N$ limit through integro-differential equations for the correlation function, $C(t,t')=\lim_{N\to \infty} \sum_i\langle x_i(t)x_i(t')\rangle/N$, the response function $R(t,t')=\lim_{N\to \infty} \frac1N\sum_i\frac{d\langle x_i(t)\rangle}{d\eta_i(t')}$ and the magnetization  $\Cmag(t)=\lim_{N\to \infty} \sum_i\langle x_i(t)x_i^*\rangle /N$. 

To obtain these equations we use the techniques developed in the context of mean-field spin glass systems \cite{MPV87, Cu03}. 
We call $\eta_i(t)$ a time dependent noise and we indicate with $\langle \cdot \rangle$ the average with respect to it. The noise is Gaussian and characterized by $\langle \eta_i(t)\rangle=0$ for all $t$ and $i=1,\ldots N$ and $\langle \eta_i(t) \eta_j(t')\rangle = 2\delta_{ij} \delta(t-t')$. As before we will denote by $\mathbb{E}[\dots]$ the average with respect to the realization of disorder that in this case goes back to the specific realization of the signal. 

Before proceeding, it is useful to introduce a set of auxiliary variables that will help in the following. 
For  $k\in\{2,p\}$ we define $r_k \equiv r_k(t) = 2/\left(kT_k(t)\Delta_k\right)$, $f_k(x)=x^k/2$ and $m(t)\doteq\frac1N\sum_ix_i(t)x_i^*$, and the random variable $\tilde{\xi}_{i_1\dots i_k}\equiv \frac1{\Delta_k}\xi_{i_1\dots i_k} \sim \mathcal{N}(0,1/\Delta_k)$. The time dependence in $T_k$, will be used in the smart annealing protocol that will be used to avoid part of the Langevin hard phase. 
We introduce a time dependent Hamiltonian
\begin{equation*}
	\begin{split}
		\mathcal{H}(t) &= -\frac1{T_2(t)\sqrt{N}}\sum_{i<j}\tilde{\xi}_{ij}x_i(t)x_j(t) -\frac{\sqrt{(p-1)}!}{T_p(t)N^{\frac{p-1}2}}\sum_{i_1<\dots<i_p}\tilde{\xi}_{i_1\dots i_p}x_{i_1}(t)\dots x_{i_p}(t) \\
		&- Nr_2(t)f_2(m(t)) - Nr_p(t)f_p(m(t))\,,
	\end{split} \label{time_hamiltonian}
\end{equation*}
and the associated Langevin dynamics
\begin{equation}\label{lng}
    \begin{split}
        \dot{x}_i(t) &=-\mu(t) x_i(t) -\frac{\partial \mathcal{H}}{\partial x_i}(t) - \eta_i(t) = -\mu(t) x_i(t) -\frac1{T_2(t)\sqrt{N}}\sum_{j(\neq i)}\tilde{\xi}_{ij}x_j(t)+
        \\
        &+ r_2(t)f'_2(m(t))-\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(i,i_1,\dots ,i_{p-1})\setminus i}\tilde{\xi}_{ii_1\dots i_{p-1}}x_{i_1}(t)\cdots x_{i_{p-1}}(t)+r_p(t)f'_p(m(t)) - \eta_i(t)\,,
    \end{split}
\end{equation}
with $\mu$ a Langrange multiplier that enforces the spherical constraint $\sum_{i=1}^N x_i^2(t)=N$.
If $T_k(t)=1$ for all $k=2,\ p$, the stationary equilibrium distribution for the Langevin dynamics is given by the posterior measure. 
Using Ito's lemma one finds 
\[
\frac 1 N\frac{d}{dt}\sum_i x_i^2(t)=\frac 2 N\sum_i x_i(t)
\dot{x}_i(t)+2 \, . 
\]
Since the spherical constraint imposes the left-hand-side to be zero, one obtains a condition on the right-hand-side. By plugging the expression (\ref{lng}) in it, one gets that in the large $N$ limit 
\begin{equation}
	\mu(t) = 1 - 2 \mathcal{H}_2(t) - p \mathcal{H}_p(t)
\end{equation}
where
\begin{equation}
{\cal H}_k = -\frac{\sqrt{(k-1)}!}{T_k(t)N^{\frac{k-1}2}}\sum_{i_1<\dots<i_k}\tilde{\xi}_{i_1\dots i_k}x_{i_1}(t)\dots x_{i_k}(t)- Nr_k(t)f_k(m(t))\ \ \ \ \ \ k=2,p
\end{equation}
are the parts of the Hamiltonian defined in Eq.~(\ref{time_hamiltonian}) relative to the matrix ($k=2$) and to the tensor ($k=p$).

Note that we have not specified any initial condition for the variables $x_i(t=0)$. Therefore, since we always employ the spherical constraint, the initial condition for the dynamics is a point on the $N$ dimensional hypersphere $|x|^2=N$ extracted with the flat measure. 

In order to analyze the Langevin dynamics in the large $N$ limit, we will use the dynamical cavity method \cite{MPV87, CC05, agoritsas2018out}. We will consider a system of $N$ variables, with $N\gg1$, and add a new one. This new variable will be considered as a small perturbation to the original system but at the same time will be treated self consistently. 
%To leading order in $N$ the old spins will be linearly perturbed, we can substitute the dynamical equation of the old spins with the linear term into the dynamical equation of the new spin. The resulting dynamics can be then split into two major contributions a stochastic one and a deterministic one. Being a linear functional of Gaussian random variables, the stochastic term will behave as a Gaussian random variable as well, and therefore it can be characterized by the first two moments. The second, deterministic, term will give a simple expression after some algebra. As result we will obtain the dynamical equation of a single spin system that contains a noise with a complicated variance structure. This expression allows to evaluate interesting variables, the protagonists introduced in the previous section: $C(t,t')$, $R(t,t')$ and $\Cmag(t)$.   


\subsection{Dynamical Mean-Field Equations}
In the following we will drop the time dependence for simplicity restoring it only when it is needed. 
Given the system with $N$ variables $i=1\dots N$, we add a new one, say $i=0$, and define $\tilde{m}=\frac1{N+1}\sum_{i=0}^Nx_ix_i^*\simeq\frac1N\sum_{i=0}^Nx_ix_i^*$ (henceforth we use the symbol $\simeq$ to denote two quantities that are 
equal up to terms that vanish in the large-$N$ limit).
The Langevin equation associated to the new variable is
\begin{equation}
    \begin{split}
        \dot{x}_0 &=-\mu x_0 -\frac1{T_2(t)\sqrt{N}}\sum_{j(\neq 0)}\tilde{\xi}_{0j}x_j+r_2f'_2(\tilde{m})-\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}x_{i_1}\cdots x_{i_{p-1}}+r_pf'_p(\tilde{m}) - \eta_0\,,
    \end{split}
\end{equation}
where we used that $N\simeq N+1$ for $N\gg 1$.
We will consider the contribution of the new variable on the others in perturbation theory. 
In the dynamical equations for the variables $i=1,\ldots, N$ we can isolate the variable $i=0$ and write
\begin{equation}
    \begin{split}
        \dot{x}_i &= -\mu x_i -\frac1{T_2(t)\sqrt{N}}\sum_{j(\neq i,0)}\tilde{\xi}_{ij}x_j+r_2f'_2(m)-\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(i,i_1,\dots ,i_{p-1})\setminus i,0}\tilde{\xi}_{ii_1\dots i_{p-1}}x_{i_1}\cdots x_{i_{p-1}}\\
        &+r_pf'_p(m) - \eta_i +H_i\,,
    \end{split}
\end{equation}
with
\begin{equation}
    H_i(t)=\left(r_2f_2''(m)+r_pf_p''(m)\right)\frac1Nx_0-\frac1{T_2(t)\sqrt{N}}\tilde{\xi}_{0i}x_0-\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(i,0,i_1,\dots ,i_{p-2})\setminus i,0}\tilde{\xi}_{i0i_1\dots i_{p-2}}x_0x_{i_1}\cdots x_{i_{p-2}}\,.
\end{equation}
Consider the unperturbed variables $x_i^0=x_i\big|_{H_i=0}$. At leading order in $N$ we can write
\begin{equation}
x_i\simeq x_i^0+\int_{t_o}^tdt'\frac{\delta x_i(t)}{\delta H_i(t')}\bigg|_{H_i=0}H_i(t')\:.
\end{equation}
 In the dynamical equation for the variable 0 we can identify a piece associated to the unperturbed variables $x_i^0$. This term can be thought of collectively  as a stochastic term $\Xi(t)$
\begin{equation}\label{eq:i0 spin perturbed}
    \begin{split}
        \dot{x}_0 &=-\mu x_0 \overbrace{-\frac1{T_2(t)\sqrt{N}}\sum_{j(\neq 0)}\tilde{\xi}_{0j}x^0_j-\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}x^0_{i_1}\cdots x^0_{i_{p-1}} - \eta_0}^{\doteq\;\Xi(t)}+\\
        &+r_2f'_2(m)+r_pf'_p(m)+\left(r_2f_2''(m)+r_pf_p''(m)\right)\frac1Nx_0-\frac1{T_2(t)\sqrt{N}}\sum_{j(\neq0)}\tilde{\xi}_{0j}\int_{t_o}^tdt'\frac{\delta x_j(t)}{\delta H_j(t')}\bigg|_{H_j=0}H_j(t')+\\
        &-\Bigg[\frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}\int_{t_o}^tdt'\frac{\delta x_{i_1}(t)}{\delta H_{i_1}(t')}\bigg|_{H_{i_1}=0}H_{i_1}(t')x^0_{i_2}\cdots x^0_{i_{p-1}}+\text{permutations}\Bigg]\,.
    \end{split}
\end{equation}
Indeed $\Xi(t)$ encodes the effect of a kind of bath made by of the unperturbed variables $i=1,\ldots, N$ to the new one. 
We can show that at leading order in $N$, $\Xi(t)$ is a Gaussian noise with zero mean and variance given by
\begin{equation*}
    \begin{split}
        \mathbb{E}\langle \Xi(t)\Xi(t')\rangle  &= 2\delta(t-t')-\mathbb{E}\left[ \frac1{T_2(t)T_2(t')N}\sum_{j(\neq0)}\sum_{l(\neq0)}\tilde{\xi}_{0j}\tilde{\xi}_{0l}x_j^0(t)x_l^0(t')\right] +\\
        &-\mathbb{E}\left[ \frac{(p-1)!}{T_p(t)T_p(t')N^{p-1}}\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\sum_{(0,j_1,\dots ,j_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}\tilde{\xi}_{0j_1\dots j_{p-1}}x^0_{i_1}\cdots x^0_{i_{p-1}}x^0_{j_1}\cdots x^0_{j_{p-1}}\right]
    \end{split} 
\end{equation*}
and the second term can be simplified as
\begin{equation*}
    \begin{split}
       \mathbb{E}\Bigg[ & \frac{(p-1)!}{T_p(t)T_p(t')N^{p-1}} \sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\sum_{(0,j_1,\dots ,j_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}\tilde{\xi}_{0j_1\dots j_{p-1}}x^0_{i_1}\cdots x^0_{i_{p-1}}x^0_{j_1}\cdots x^0_{j_{p-1}}\Bigg]  =\\
        &\simeq \frac{(p-1)!}{N^{p-1}}\frac1{T_p(t)T_p(t')\Delta_p} \sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\langle x^0_{i_1}(t)x^0_{i_1}(t')\cdots x^0_{i_{p-1}}(t)x^0_{i_{p-1}}(t')\rangle =\frac1{T_p(t)T_p(t')\Delta_p}C^{p-1}(t,t')\,,
    \end{split} 
\end{equation*}
where we used $\sum_{(i_1,\dots,i_k)}=\frac1{k!}\sum_{1\le i_1,\dots,i_k\le N}$, we neglected terms sub-leading in $N$, and we used the definition of the dynamical correlation function
\begin{equation}
\nonumber
C(t,t') = \frac 1N \sum_{i=1}^N \langle x_i(t) x_i(t')\rangle \:.
\end{equation}
Therefore we have
\begin{align}
    &\mathbb{E}\langle \Xi(t)\rangle =0\,;\\
    &\mathbb{E}\langle \Xi(t)\Xi(t')\rangle =2\delta(t-t')+\frac1{T_2(t)T_2(t')}C(t,t')+\frac1{T_p(t)T_p(t')\Delta_p}C^{p-1}(t,t')\,.
\end{align}
Now we can focus of the deterministic term coming from the first order
perturbation in \eqref{eq:i0 spin perturbed}. Consider just the
integral for the $p$-body term, the other will be given by setting
$p=2$
\begin{equation}\label{eq:i0 deterministic perturbation}
    \begin{split}
        \frac{\sqrt{(p-1)!}}{T_p(t)N^{\frac{p-1}2}}&\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\tilde{\xi}_{0i_1\dots i_{p-1}}\int_{t_o}^tdt'\frac{\delta x_{i_1}(t)}{\delta H_{i_1}(t')}\bigg|_{H_{i_1}=0}H_{i_1}(t')x^0_{i_2}\cdots x^0_{i_{p-1}}+\text{permutations}=\\
        &\simeq \frac{(p-1)!}{T_p(t)N^{p-1}}\sum_{(0,i_1,\dots ,i_{p-1})\setminus 0}\tilde{\xi}^2_{0i_1\dots i_{p-1}}\int_{t_o}^tdt'\frac1{T_p(t')}\frac{\delta x_{i_1}(t)}{\delta H_{i_1}(t')}\bigg|_{H_{i_1}=0} x^0_{i_1}(t)x^0_{i_1}(t')\cdots x^0_{i_{p-2}}(t)x^0_{i_{p-2}}(t')x_0(t')+\\
        &+\text{permutations} \simeq -\frac{p-1}{T_p(t)\Delta_p}\int_{t_o}^tdt'\frac1{T_p(t')}R(t,t')C^{p-2}(t,t')x_0(t')
    \end{split}
\end{equation}
where we have used the definition of the response function
\begin{equation}\nonumber
R(t,t') = \frac{1}{N} \sum_{i=1}^N \left\langle \frac{\delta x_i(t)}{\delta H_i(t')}\right \rangle \:.
\end{equation}
Plugging \eqref{eq:i0 deterministic perturbation} into \eqref{eq:i0 spin perturbed} we obtain an effective dynamical equation for the new variable in terms of the correlation and response function
of the system with $N$ variables
\begin{equation}\label{eq:i0 spin}
    \begin{split}
        \dot{x}_0(t)&=-\mu(t) x_0(t)+\Xi(t)+r_pf_p'(\Cmag(t))+r_2f_2'(\Cmag(t))+
        \\
        &+\frac{p-1}{T_p(t)\Delta_p}\int_{t_o}^tdt''\frac1{T_p(t'')}R(t,t'')C^{p-2}(t,t'')x_0(t'')+\frac1{T_2(t)\Delta_2}\int_{t_o}^tdt''\frac1{T_p(t'')}R(t,t'')x_0(t'')\,.
    \end{split}
\end{equation}
In order to close Eq.~(\ref{eq:i0 spin}) we need to give the recipe to compute the correlation and response function.

\subsection{Integro-differential equations}
In order to obtain the final equations for dynamical order parameters we will assume that the new variable $x_0$ is a typical one, namely it has the same statistical nature of all the others. 
Therefore we can assume that 
\begin{equation}
\begin{split}
C(t,t')&\doteq \mathbb{E}\langle x_0(t)x_0(t')\rangle\\
R(t,t')&\doteq \mathbb{E}\left\langle \frac{\delta x_0(t)}{\delta \Xi(t')}\right\rangle\\
\Cmag(t)&\doteq \mathbb{E}\langle x_0(t)x_0^*\rangle\:.
\end{split}
\label{closure}
\end{equation}

Eqs.~(\ref{closure}) give a way to obtain the equation for all the correlation functions. 
Indeed we can consider Eq.~(\ref{eq:i0 spin}), multiply it by $x_0(t')$, or differentiate it with respect to an external field $h_0(t')$,  or multiply it it by $x_0^*$ and we can average the results over the disorder and thermal noise.
Using the following identity
\begin{equation}\label{eq:Xi x0 covariance}
    \begin{split}
        \mathbb{E}\langle \Xi(t) & x_0(t')\rangle =\int\mathcal{D}\Xi(t)\;\Xi(t)x_0(t')e^{-\int d\bar{t}d\tilde{t}\Xi(\bar{t})\mathbb{K}^{-1}(\bar{t},\tilde{t})\Xi(\tilde{t})}=\\
        &=-\int dt'' \int\mathcal{D}\Xi(t)\;x_0(t')\frac{\delta}{\delta\Xi(t'')}e^{-\int d\bar{t}d\tilde{t}\Xi(\bar{t})\mathbb{K}^{-1}(\bar{t},\tilde{t})\Xi(\tilde{t})} \mathbb{K}(t,t'')=\\
        &=\int dt''\mathbb{E}\left\langle \frac{\delta x_0(t')}{\delta \Xi(t'')}\mathbb{K}(t,t'')\right\rangle =\int dt''R(t',t'')\mathbb{K}(t,t'')=\\
        &=2R(t',t)+\frac1{T_p(t)\Delta_p}\int_{t_o}^{t'}dt''\frac1{T_p(t'')}R(t',t'')C^{p-1}(t,t'')+\frac1{T_2(t)\Delta_2}\int_{t_o}^{t'}dt''\frac1{T_2(t'')}R(t',t'')C(t,t'')
    \end{split}
\end{equation}
we get the following Langevin State Evolution (LSE) equations
    \begin{align}
        \begin{split} 
\label{eq:dynamic correlation}
            \frac{\partial}{\partial t}C(t,t')&= \mathbb{E}\langle \dot{x}_0(t)x_0(t')\rangle = 2R(t',t)-\mu(t)C(t,t')+r_p(t)f_p'(\Cmag(t))\Cmag(t')+r_2(t)f_2'(\Cmag(t))\Cmag(t')+\\
            &+(p-1)\frac1{T_p(t)\Delta_p}\int_{t_o}^tdt''\frac1{T_p(t'')}R(t,t'')C^{p-2}(t,t'')C(t',t'')+\\
            &+\frac1{T_p(t)\Delta_p}\int_{t_o}^{t'}dt''\frac1{T_p(t'')}R(t',t'')C^{p-1}(t,t'')+\\
            &+\frac1{T_2(t)\Delta_2}\int_{t_o}^tdt''\frac1{T_2(t'')}R(t,t'')C(t',t'')+\frac1{T_2(t)\Delta_2}\int_{t_o}^{t'}dt''\frac1{T_2(t'')}R(t',t'')C(t,t'')\,; 
        \end{split} \\
          \begin{split} 
\label{eq:dynamic response function}
            \frac{\partial}{\partial t}R(t,t')&=\mathbb{E}\left\langle \frac{\delta \dot{x}_0(t)}{\delta\Xi(t')}\right\rangle =\\
            &=\delta(t-t')-\mu(t)R(t,t')+(p-1)\frac1{T_p(t)\Delta_p}\int_{t'}^tdt''\frac1{T_p(t'')}R(t,t'')R(t'',t')C^{p-2}(t,t'')+\\
            &+\frac1{T_2(t)\Delta_2}\int_{t'}^tdt''\frac1{T_2(t'')}R(t,t'')R(t'',t')\,;
        \end{split} \\
       \begin{split}  
\label{eq:dynamic magnetization}
            \frac{\partial}{\partial t}\Cmag(t)&=\mathbb{E}\langle \dot{x}_0(t)x^*_0\rangle = 
            \\
            &=-\mu(t)\Cmag(t)+r_p(t)f_p'(\Cmag(t))+r_2(t)f_2'(\Cmag(t))+\\
            &+(p-1)\frac1{T_p(t)\Delta_p}\int_{t_o}^tdt''\frac1{T_p(t'')}R(t,t'')C^{p-2}(t,t'')\Cmag(t'')+\frac1{T_2(t)\Delta_2}\int_{t_o}^tdt''\frac1{T_2(t'')}R(t,t'')\Cmag(t'')\,;
        \end{split} \\
\label{eq:dynamic mu}
        \begin{split}
            \mu(t)&=1+r_p(t)f_p'(\Cmag(t))\Cmag(t)+r_2(t)f_2'(\Cmag(t))\Cmag(t)+\\
            &+p\frac1{T_p(t)\Delta_p}\int_{t_o}^tdt''\frac1{T_p(t'')}R(t,t'')C^{p-1}(t,t'')+2\frac1{T_2(t)\Delta_2}\int_{t_o}^tdt''\frac1{T_2(t'')}R(t,t'')C(t,t'')\,.
        \end{split}
    \end{align}
Note that the last equation for $\mu(t)$ is obtained by imposing the spherical constraint $C(t,t)=1\;\forall t$ using the fact that $0 = \frac{dC(t,t)}{dt} = \frac{\partial C(t,t')}{\partial t}\Big|_{t'=t} + \frac{\partial C(t',t)}{\partial t}\Big|_{t'=t}$. The boundary conditions of this equations are: $C(t,t)=1$ the spherical constrain, $R(t,t)=0$ which comes from causality in the It\^{o} approach and $R(t,t'\to t^-)=1$. 
The initial condition for $\Cmag(0)=\Cmag_0$ is the overlap with the initial configuration with the true signal. 
If the initial configuration is random, $\Cmag_0=0$ but will have finite size fluctuations, as in the case of AMP. 
Therefore we can think that $\Cmag_0=\epsilon$ being $\epsilon$ an arbitrary small positive number. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical solution of the LSE equations}
\label{section:numerical implementation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The dynamical equations (\ref{eq:dynamic correlation}-\ref{eq:dynamic response function}-\ref{eq:dynamic magnetization}-\ref{eq:dynamic mu}) were integrated numerically using two schemes:
\begin{itemize}
	\item fixed time-grid: the derivatives were discretized and integrated according to their causal structure. This method is suited only for short times (up to $500$ time units);
	\item dynamic time-grid: the step size is doubled after a given number of steps and the equations are solved self-consistently for every waiting-time. This is the approach proposed in \cite{kim2001dynamics} and described in Appendix C of \cite{berthier2007spontaneous}. It allows integration up to very large times (up to $10^6$ time units).
\end{itemize}

The results of these algorithms are concisely reported in the phase diagram shown in the main paper. In what follows we will present the algorithms and a series of investigations that we carried out to check their stability, we will explain the procedure followed to delimit the Langevin hard region, and we will discuss how we can enter into part of that region by choosing a proper annealing protocol. The codes are available online \cite{LSEcode}.


\subsection{Fixed time-grid $(2+p)$-spin}\label{sec:numerical implementation - fixed grid}

In this approach time-derivatives and integrals were discretized using $\frac{\partial}{\partial t}f(t,t') \simeq \frac1{\Delta t}\left[f(t+\Delta t,t')-f(t,t')\right]$, and the trapezoidal rule for integration $\int_0^t f(t)dt \simeq \frac{\Delta t}2 \sum_{l=0}^{t/\Delta t-1} \left[f(l\Delta t)+f((l+1)\Delta t)\right]$.
For instance we defined a function for computing the update in the the
response function, \eqref{eq:dynamic response function} as follows
\begin{equation*}
	\begin{split}
		R(t +\Delta t &,t') = R(t,t') -\Delta t\,\mu(t)R(t,t') + \frac12\frac{\Delta t^2}{\Delta_2} \sum_{l=t'/\Delta t}^{t/\Delta t-1} \left[R(t,l\Delta t)R(l\Delta t,t')+R(t,(l+1)\Delta t)R((l+1)\Delta t,t')\right] +\\
		&+ (p-1)\frac{\Delta t^2}{\Delta_p} \sum_{l=t'/\Delta t}^{t/\Delta t-1}\left[C^{p-2}(t,l\Delta t)R(t,l\Delta t)R(l\Delta t,t')+C^{p-2}(t,(l+1)\Delta t)R(t,(l+1)\Delta t)R((l+1)\Delta t,t')\right]\;.
	\end{split}
\end{equation*} 
Analogously we defined the other integrators. A simple causal
integration scheme, being careful with the It\^o prescription, gives the
pseudo-code below.
\begin{algorithmic}
	\STATE $C(0,0) \gets1$;  $R(0,0) \gets0$;  $\Cmag(0) \gets \Cmag_0$;
	\FOR {$t \le t_{\max}$}
		\STATE $C(t+\Delta t,t+\Delta t) \gets1$;  $R(t+\Delta t,t+\Delta t) \gets0$;
		\STATE $\mu(t) \gets $ compute\_mu($C$, $R$, $\Cmag$, $t$);
		\STATE $\Cmag(t+\Delta t) \gets$ compute\_mag($\mu$, $C$, $R$, $\Cmag$, $t$);
		\FOR {$t' \le t$} 
        	\STATE $C(t+\Delta t,t') \gets$ compute\_C($\mu$, $C$, $R$, $\Cmag$, $t$);
        	\STATE $R(t+\Delta t,t') \gets$ compute\_R($\mu$, $C$, $R$, $\Cmag$, $t$);
		\ENDFOR
		\STATE $R(t+\Delta t,t) \gets1$;
	\ENDFOR
\end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dynamical time-grid $(2+p)$-spin}

\begin{figure}[H]
    \centering
    \subfigure[Memory allocation;]{
        \includegraphics[scale=.5]{img/{KL_algo_1}.pdf}
    }
    \subfigure[step 1;]{
        \includegraphics[scale=.5]{img/{KL_algo_2}.pdf}
    }
    \subfigure[step 2;]{
        \includegraphics[scale=.5]{img/{KL_algo_3}.pdf}
    }
    \subfigure[step 3;]{
        \includegraphics[scale=.5]{img/{KL_algo_4}.pdf}
    }\\
    \centering
    \subfigure[step 4.1;]{
        \includegraphics[scale=.5]{img/{KL_algo_5}.pdf}
    }
    \subfigure[step 4.2;]{
        \includegraphics[scale=.5]{img/{KL_algo_6}.pdf}
    }
    \subfigure[step 2;]{
        \includegraphics[scale=.5]{img/{KL_algo_7}.pdf}
    }
    \subfigure[step 3.]{
        \includegraphics[scale=.5]{img/{KL_algo_8}.pdf}
    }
    \caption{Representation of the initialization and the first two iterations for the evaluation of a two-times observable using the dynamic-grid algorithm. The empty circles represent slots allocated in memory but not associated to any specific value, while the full circles are memory slots already associated. For any two time function, it first allocates the memory (a), than it fills half of the grid by linear propagation (b). Still using linear propagation it fills the slots with $t-t'\ll1$ (c), and it sets the other values by imposing self-consistency (d). Finally it halves the grid (e), doubles time step and it allocates the memory (f). Then the algorithm loops following the same scheme as in (b-c-d-e).}
    \label{fig:algorithm KL}
\end{figure}
The numerical scheme we are going to discuss is presented in the Bayes-Optimal case where $T_2(t) \equiv T_p(t) \equiv 1$. However the derivation that we propose can be easily generalized to the case where the $T$s assume different values, but are constants\footnote{Therefore we do not employ this algorithm to solve the LSE equations in the smart annealing protocol for which instead we use the fixed time-grid algorithm.}. It is convenient to manipulate the equations to obtain an equivalent set of equations for the functions $C(t,t')$, $Q(t,t') \doteq 1 - C(t,t') - \int_{t'}^t R(t,t'')dt''$, $\Cmag(t)$, where $Q(t,t')$ represents the deviation from Fluctuation Dissipation Theorem (FDT) at time $t$ starting from time $t'$. 
Indeed when the FDT theorem holds, it states that $R(t,t') = -\partial_t C(t,t')$.

We briefly anticipate the strategy that the algorithm uses to solve the equations. The algorithm discretizes the times into $N_t$ intervals, first starting from the boundary conditions, $C(t,t) = 1$, $Q(t,t) = 0$ and $\Cmag = \Cmag_0\in[0;1]$, it fills the grid for small times (or small time differences $\tau=t-t'\ll1$) using linear propagation. Given a time $t$ and the initial guess for the Lagrange multiplier obtained by the linear propagator, the integrals are discretized and evaluated, then the results is used to update the value of the Lagrange multiplier. This procedure is repeated iteratively until convergence. Once that the first grid is filled, it follows a coarse-graining procedure where the sizes of the time intervals is doubled and only half of the information is retained. This procedure is repeated a fixed number of doubling of the original grid. The doubling scheme allows to explore exponentially long times at the cost of loosing part of the information, the direct consequence of this is the loss of stability for very large times (especially when the functions $C(t,t')$, $R(t,t')$, $\Cmag(t)$ undergo fast changes at large times).

\paragraph{Dynamical equations in the algorithm.} We recall the function $f_k(x) = \frac{x^k}2$ and its derivatives, $f_k'(x) = \frac{kx^{k-1}}2$ and $f_k''(x) = \frac{k(k-1)x^{k-2}}2$. For simplicity in the notation, we introduce also $f_k(t,t') \doteq f_k\left(C(t,t')\right)$
\begin{align*}
        (\partial_t+\mu(t))C(t,t') &= 2R(t',t)+r_2\Cmag(t')f_2'(\Cmag(t))+r_p\Cmag(t')f_p'(\Cmag(t))+\\
        &+\frac1{\Delta_2}\int_0^{t'}dt''f_2'(t,t'')R(t',t'')+\frac1{\Delta_2}\int_0^{t}dt''f_2''(t,t'')R(t,t'')C(t',t'')+\\
        &+\frac2{p\Delta_p}\int_0^{t'}dt''f_p'(t,t'')R(t',t'')+\frac2{p\Delta_p}\int_0^{t}dt''f_p''(t,t'')R(t,t'')C(t',t'')\,,
        \\
        (\partial_t+\mu(t))R(t,t') &= \delta(t-t')+\frac1{\Delta_2}\int_{t'}^t dt''f_2''(t,t'')R(t,t'')R(t'',t')+\\
        &+\frac2{p\Delta_p}\int_{t'}^t dt''f_p''(t,t'')R(t,t'')R(t'',t')\,,
        \\
        (\partial_t+\mu(t))\Cmag(t) &=r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))+\\
        &+\frac1{\Delta_2}\int_0^tdt''f_2''(t,t'')R(t,t'')\Cmag(t'')+\frac2{p\Delta_p}\int_0^tdt''f_p''(t,t'')R(t,t'')\Cmag(t'')\,,
        \\
        \mu(t) &= 1+r_2\Cmag(t)f_2'(\Cmag(t))+r_p\Cmag(t)f_p'(\Cmag(t))+\\
        &+\frac2{\Delta_2}\int_0^tdt''f_2'(t,t'')R(t,t'')+\frac2{\Delta_p}\int_0^tdt''f_p'(t,t'')R(t,t'')\,.
\end{align*}
Following the lines of \cite{berthier2007spontaneous}, we introduce the FDT violation function, $Q(t,t')$, and after some manipulation the systems becomes
\begin{align}\label{eq:sys for numerics}
	\begin{split}
        (\partial_t+ &\mu(t))C(t,t') = \Cmag(t')\left[r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))\right]+\\
        &+\frac1{\Delta_2}\Big\{\int_0^{t'}dt''\left[f_2'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]+\\
        &-\int_{t'}^{t}dt''\left[f_2'(t,t'')\frac{\partial C(t'',t')}{\partial t''}-f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t'',t')\right]+f_2'(1)C(t,t')-f_2'(t,0)C(t',0)\Big\}+\\
        &+\frac2{p\Delta_p}\Big\{\int_0^{t'}dt''\left[f_p'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]+\\
        &-\int_{t'}^{t}dt''\left[f_p'(t,t'')\frac{\partial C(t'',t')}{\partial t''}-f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t'',t')\right]+f_p'(1)C(t,t')-f_p'(t,0)C(t',0)\Big\}\,,
	\end{split}
    \\
	\begin{split}
        (\partial_t+ &\mu(t))Q(t,t') = \mu(t)-1+\frac1{\Delta_2}\Big\{-\int_{t'}^t dt''f_2'(t,t'')\frac{\partial Q(t'',t')}{\partial t''}+\int_{t'}^t dt''f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}[Q(t'',t')-1]+\\
        &+f_2'(1)[Q(t,t')-1]+f_2'(t,0)C(t',0)-\int_0^{t'}dt''\left[f_2'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]\Big\}+\\
        &+\frac2{p\Delta_p}\Big\{-\int_{t'}^t dt''f_p'(t,t'')\frac{\partial Q(t'',t')}{\partial t''}+\int_{t'}^t dt''f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}[Q(t'',t')-1]+\\
        &+f_p'(1)[Q(t,t')-1]+f_p'(t,0)C(t',0)-\int_0^{t'}dt''\left[f_p'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]\Big\}+\\
        &-\Cmag(t')\left[r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))\right]\,,
	\end{split}
    \\
	\begin{split}
        (\partial_t+ &\mu(t))\Cmag(t) = r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))+\frac1{\Delta_2}\Big\{f_2'(1)\Cmag(t)-f_2'(t,0)\Cmag(0)
        -\int_0^tdt''f_2'(t,t'')\frac{d}{d t''}\Cmag(t'')+\\
        &+\int_0^tdt''f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}\Cmag(t'')\Big\}+\frac2{p\Delta_p}\Big\{f_p'(1)\Cmag(t)-f_p'(t,0)\Cmag(0)-\int_0^tdt''f_p'(t,t'')\frac{d}{d t''}\Cmag(t'')+\\
        &+\int_0^tdt''f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}\Cmag(t'')\Big\}\,,
	\end{split}
    \\
	\begin{split}
        \mu(t) &= 1+r_2\Cmag(t)f_2'(\Cmag(t))+r_p\Cmag(t)f_p'(\Cmag(t))+\frac2{\Delta_2}[f_2(1)-f_2(t,0)]+\frac2{\Delta_p}[f_p(1)-f_p(t,0)]+\\
        &+\int_0^tdt''\left[\frac2{\Delta_2}f_2'(t,t'')+\frac2{\Delta_p}f_p'(t,t'')\right]\frac{\partial Q(t,t'')}{\partial t''}\,,
	\end{split}
\end{align}
further simplifications can be obtained introducing $\mu'(t)=\mu(t)-\frac2{\Delta_2}f_2(1)-\frac2{\Delta_p}f_p(1)$
\begin{align}\label{eq:sys for numerics mu'}
	\begin{split}
        \mu'(t) &= 1+r_2\Cmag(t)f_2'(\Cmag(t))+r_p\Cmag(t)f_p'(\Cmag(t))-\frac2{\Delta_2}f_2(t,0)-\frac2{\Delta_p}f_p(t,0)+\\
        &+\int_0^tdt''\left[\frac2{\Delta_2}f_2'(t,t'')+\frac2{\Delta_p}f_p'(t,t'')\right]\frac{\partial Q(t,t'')}{\partial t''}\,,
	\end{split}
    \\
	\begin{split}
        (\partial_t+ &\mu'(t))C(t,t') = \Cmag(t')\left[r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))\right]+\\
        &+\frac1{\Delta_2}\Big\{\int_0^{t'}dt''\left[f_2'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]+\\
        &-\int_{t'}^{t}dt''\left[f_2'(t,t'')\frac{\partial C(t'',t')}{\partial t''}-f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t'',t')\right]-f_2'(t,0)C(t',0)\Big\}+\\
        &+\frac2{p\Delta_p}\Big\{\int_0^{t'}dt''\left[f_p'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]+\\
        &-\int_{t'}^{t}dt''\left[f_p'(t,t'')\frac{\partial C(t'',t')}{\partial t''}-f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t'',t')\right]-f_p'(t,0)C(t',0)\Big\}\,,
	\end{split}
    \\
	\begin{split}
        (\partial_t+ &\mu'(t))Q(t,t') = \mu'(t)-1-\Cmag(t')\left[r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))\right]+\\
        &+\frac1{\Delta_2}\Big\{-\int_{t'}^t dt''f_2'(t,t'')\frac{\partial Q(t'',t')}{\partial t''}+\int_{t'}^t dt''f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}[Q(t'',t')-1]+\\
        &+f_2'(t,0)C(t',0)-\int_0^{t'}dt''\left[f_2'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]\Big\}+\\
        &+\frac2{p\Delta_p}\Big\{-\int_{t'}^t dt''f_p'(t,t'')\frac{\partial Q(t'',t')}{\partial t''}+\int_{t'}^t dt''f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}[Q(t'',t')-1]+\\
        &+f_p'(t,0)C(t',0)-\int_0^{t'}dt''\left[f_p'(t,t'')\frac{\partial Q(t',t'')}{\partial t''}+f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}C(t',t'')\right]\Big\}\,,
	\end{split}
    \\
	\begin{split}
        (\partial_t+ &\mu'(t))\Cmag(t) = r_2f_2'(\Cmag(t))+r_pf_p'(\Cmag(t))+\frac1{\Delta_2}\Big\{-f_2'(t,0)\Cmag(0)+\\
        &-\int_0^tdt''f_2'(t,t'')\frac{d}{d t''}\Cmag(t'')+\int_0^tdt''f_2''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}\Cmag(t'')\Big\}+\\
        &+\frac2{p\Delta_p}\Big\{-f_p'(t,0)\Cmag(0)+\\
        &-\int_0^tdt''f_p'(t,t'')\frac{d}{d t''}\Cmag(t'')+\int_0^tdt''f_p''(t,t'')\frac{\partial Q(t,t'')}{\partial t''}\Cmag(t'')\Big\}\,.
	\end{split}
\end{align}
\paragraph{First order expansion coefficients.} In the numerics we will initialize the grid by a linear propagation of the initial conditions. To determine the coefficients to use we can expand the functions up the second term for small values of $\tau$ (and in the last equation of $t$)
\begin{equation}
    \begin{split}
        C(t'+\tau,t')&=C(t',t')+C^{(1,0)}(t',t')\tau+\frac12C^{(2,0)}(t',t')+O(\tau^3)\,
        , \\
        Q(t'+\tau,t')&=Q(t',t')+Q^{(1,0)}(t',t')\tau+\frac12Q^{(2,0)}(t',t')+O(\tau^3)\,
        , \\
        \Cmag(t)&=\Cmag(0)+\Cmag^{(1)}(0)\tau+\frac12\Cmag^{(2)}(0)+O(t^3)
        \, . 
    \end{split}
\end{equation}
This gives the following coefficients: $C(t,t)=1$, $C^{(1,0)}(t,t)=-1$, $Q(t,t)=0$, $Q^{(1,0)}(t,t)=0$, $\Cmag(0)=\Cmag_0$ and $\Cmag^{(1)}(0)=\left[r_2f_2'(\Cmag_0)+r_pf_p'(\Cmag_0)\right](1-(\Cmag_0)^2)-\Cmag_0$, where $\Cmag_0$ is the initial value of the overlap with the signal.

\paragraph{Numerical integration and derivation.} The set of equations derived above presents six types of integrals
\begin{align*}
        &I_{ij}^{(1AB)}=\int_{t_j}^{t_i}dt''A(t_i,t'')\frac{\partial B(t'',t_j)}{\partial t''}\,;\\
        &I_{ij}^{(2ABC)}=\int_{t_j}^{t_i}dt''A(t_i,t'')\frac{\partial B(t_i,t'')}{\partial t''}C(t'',t_j)\,;\\
        &I_{ij}^{(3AB)}=\int_{0}^{t_j}dt''A(t_i,t'')\frac{\partial B(t_i,t'')}{\partial t''}\,;\\
        &I_{ij}^{(4ABC)}=\int_{0}^{t_j}dt''A(t_i,t'')\frac{\partial B(t_i,t'')}{\partial t''}C(t_j,t'')\,;\\
        &I_{i}^{(5AB)}=\int_{0}^{t_i}dt''A(t_i,t'')\frac{\partial B(t'')}{\partial t''}\,;\\
        &I_{i}^{(6ABC)}=\int_{0}^{t_i}dt''A(t_i,t'')\frac{\partial B(t_i,t'')}{\partial t''}C(t'')\,.
\end{align*}
The integrals can be easily discretized
\begin{align*}
    I_{ij}^{(2ABC)}&=\sum_{t_l=t_j+\delta t}^{t_i}\int_{t_l-\delta t}^{t_l}dt''A(t_i,t'')\frac{\partial B(t_i,t'')}{\partial t''}C(t'',t_j)\simeq\\
    &\simeq \sum_{t_l=t_j+\delta t}^{t_i}\int_{t_l-\delta t}^{t_l}dt_1A(t_i,t_1)\int_{t_l-\delta t}^{t_l}dt_2\frac{\partial B(t_i,t_2)}{\partial t_2}\int_{t_l-\delta t}^{t_l}dt_3C(t_3,t_j)\simeq\\
    &\simeq \sum_{t_l=t_j+\delta t}^{t_i}\frac12[A(t_i,t_l)+A(t_i,t_l-\delta t)][B(t_i,t_l)-B(t_i,t_l-\delta t)]\frac12[C(t_l,t_j)+C(t_l-\delta t,t_j)]\;.
\end{align*}
In particular the 6 integrals become
\begin{align}
	\begin{split}
        &I_{ij}^{(1AB)}=A_{im}B_{mj}-A_{ij}B_{jj}+\sum_{l=m+1}^{i}\frac12(A_{il}+A_{i(l-1)})(B_{lj}-B_{(l-1)j})+\\
        &\quad \quad \quad -\sum_{l=j+1}^{m}\frac12(B_{lj}+B_{(l-1)j})(A_{il}-A_{i(l-1)})=\\
        &\quad \quad \quad =A_{im}B_{mj}-A_{ij}B_{jj}+\sum_{l=m+1}^{i}dA_{il}^{(v)}(B_{lj}-B_{(l-1)j})-\sum_{l=j+1}^{m}(A_{il}-A_{i(l-1)})dB_{lj}^{(h)}\,;
    \end{split}
    \\
	\begin{split}
        &I_{ij}^{(2ABC)}=\sum_{l=j+1}^{i}\frac12(A_{il}+A_{i(l-1)})(B_{lj}-B_{(l-1)j})\frac12(C_{lj}+C_{(l-1)j})=\\
        &\quad \quad \quad =\sum_{l=m+1}^{i}dA_{il}^{(h)}(B_{il}-B_{i(l-1)})\frac12(C_{lj}+C_{(l-1)j})+\sum_{l=j+1}^{m}\frac12(A_{il}+A_{i(l-1)})(B_{il}-B_{i(l-1)})dC_{lj}^{(v)}\,;
	\end{split}
    \\
    &I_{ij}^{(3AB)}=A_{ij}B_{jj}-A_{i0}B_{j0}-\sum_{l=1}^{j}(A_{il}-A_{i(l-1)})dB_{jl}^{(v)}\,;
    \\
    &I_{ij}^{(4ABC)}=\sum_{l=1}^{j}\frac12(A_{il}+A_{i(l-1)})(B_{il}-B_{i(l-1)})dC_{jl}^{(v)}\,;
    \\
    &I_{i}^{(5AB)}=\sum_{l=1}^{i}dA_{il}^{(v)}(B_{l}-B_{l-1})\,;
    \\
    &I_{i}^{(6ABC)}=\sum_{l=1}^{i}\frac12(A_{il}+A_{i(l-1)})(B_{il}-B_{i(l-1)})dC_{l}\,,
\end{align}
where the superscript $(v)$ and $(h)$ represent the vertical ($t'$)
and horizontal ($t$) derivatives in the discretized times, see
Fig.~\ref{fig:algorithm KL} for an intuitive understanding.  

We also discretized the derivative using the last two time steps
\begin{equation}
    \frac{d}{dt}g(t)=\frac3{2\delta t}g(t)-\frac2{\delta t}g(t-\delta t)+\frac1{2\delta t}g(t-2\delta t)+O(\delta t^3)\,.
\end{equation}
Given the time indices $i$ and $j$, we will define and evaluate the following quantities
\begin{equation*}
    \begin{split}
        \{&C_{ij},Q_{ij},M2_{ij},N2_{ij},Mp_{ij},Np_{ij},\Cbar_i,P2_i,Pp_i,mu_i\}=\\
        &=\{C(t_i,t_j),Q(t_i,t_j),f_2'(C(t_i,t_j)),f_2''(C(t_i,t_j)),f_p'(C(t_i,t_j)),f_p''(C(t_i,t_j)),\Cmag(t_i),f_2'(\Cmag(t_i)),f_p'(\Cmag(t_i)),\mu(t_i)\}
    \end{split} 
\end{equation*}
plus the respective vertical and horizontal derivatives. 

Calling $D_i=\frac3{2dt}+\mu'_i-\frac1{\Delta_2}M2_{ii}-\frac2{p\Delta_p}Mp_{ii}$, the original dynamical equations are integrated as follow
\begin{align} \label{eq:self-consistent algo 1}
	\begin{split}
        C_{ij}D_i&= \frac2{dt}C_{(i-1)j}-\frac1{2dt}C_{(i-2)j}+\Cbar_j(r_2P2_i+r_pPp_i)+\\
        &+\frac1{\Delta_2}\left(-\dot{I}_{ij}^{(1f_2'C)}+I_{ij}^{(2f_2''QC)}+I_{ij}^{(3f_2'Q)}+I_{ij}^{(4f_2''QC)}-M2_{i0}C_{j0}\right)+\\
        &+\frac2{p\Delta_p} \left(-\dot{I}_{ij}^{(1f_p'C)}+I_{ij}^{(2f_p''QC)}+I_{ij}^{(3f_p'Q)}+I_{ij}^{(4f_p''QC)}-Mp_{i0}C_{j0}\right)\,,
	\end{split}
    \\
    \label{eq:self-consistent algo 2}
	\begin{split}
        Q_{ij}D_i&= \mu'_i-1+\frac2{dt}Q_{(i-1)j}-\frac1{2dt}Q_{(i-2)j}+\Cbar_j(r_2P2_i+r_pPp_i)+\\
        &+\frac1{\Delta_2}\left(-\dot{I}_{ij}^{(1f_2'Q)}+I_{ij}^{(2f_2''Q(Q-1))}-I_{ij}^{(3f_2'Q)}-I_{ij}^{(4f_2''QC)}-M2_{i0}C_{i0}\right)+\\
        &+\frac2{p\Delta_p} \left(-\dot{I}_{ij}^{(1f_p'Q)}+I_{ij}^{(2f_p''Q(Q-1))}-I_{ij}^{(3f_p'Q)}-I_{ij}^{(4f_p''QC)}-Mp_{i0}C_{i0}\right)\,,
	\end{split}
    \\
    \label{eq:self-consistent algo 3}
	\begin{split}
        \Cbar_iD_i&= \frac2{dt}\Cbar_{i-1}-\frac1{2dt}\Cbar_{i-2}+r_2P2_i+r_pPp_i+\\
        &+\frac1{\Delta_2}\left(-\dot{I}_i^{(5f_2'\Cbar)}+I_i^{(6f_2''Q\Cbar)}-M2_{i0}\Cbar_{0}\right)+\\
        &+\frac2{p\Delta_p} \left(-\dot{I}_i^{(5f_p'\Cbar)}+I_i^{(6f_p''Q\Cbar)}-Mp_{i0}\Cbar_{0}\right)\,.
	\end{split}
\end{align}
In the systems we used $\dot{I}$ to characterize the integrals where we remove from the sum the term present in the left-hand side (e.g. for $C_{ij}$ eq.~\ref{eq:self-consistent algo 1}).
Using Simpson's integration formula we define the increments
\begin{equation*}
	\begin{split}
    	\Delta_{il}&=\frac1{12}(Q_{il}-Q_{i(l-1)})\{W_2^2[-(M2_{i(l+1)}+N2_{i(l+1)}C_{i(l+1)})+8(M2_{il}+N2_{il}C_{il})+5(M2_{i(l-1)}+N2_{i(l-1)}C_{i(l-1)})]+\\
        &+W_p^2[-(Mp_{i(l+1)}+Np_{i(l+1)}C_{i(l+1)})+8(Mp_{il}+Np_{il}C_{il})+5(Mp_{i(l-1)}+Np_{i(l-1)}C_{i(l-1)})]\}
	\end{split}
\end{equation*}
and we determine $\mu'$ as
\begin{equation} \label{eq:self-consistent algo mu}
	\mu'=1+r_2P2_i+r_pPp_i+\delta \mu'+\sum_{l=1}^{i-N_t/4}\Delta_{il}-(W_2^2M2_{i0}+W_p^2Mp_{i0})C_{i0}\,,
\end{equation}
with $\delta \mu'$ initially set to 0.    

\paragraph{Algorithm:} Here we describe the main steps of the algorithm, pictorially represented Fig.~\ref{fig:algorithm KL}.

Discretize the time $(t,t')$ in $N_t$ (even) intervals, the results shown use $N_t = 1024$. 
\begin{enumerate}
    \item \textbf{Initialization.} Fill the first $N_t/2$ times by linear propagation of the value obtained from the perturbative analysis
        \begin{align}
                &C_{ij}=1-(i-j)dt\,;\\
                &Q_{ij}=0\,;\\
                &\Cbar_{i}=\Cmag_0+\left\{\left[r_2f_2'(\Cmag_0)+r_pf_p'(\Cmag_0)\right](1+(\Cmag_0)^2)-\Cmag_0\right\}dt\,;\\
                &M2_{ij}=f_2'(C_{ij})\,;\\
                &N2_{ij}=f_2''(C_{ij})\,;\\
                &Mp_{ij}=f_p'(C_{ij})\,;\\
                &Np_{ij}=f_p''(C_{ij})\,.
        \end{align}
    \item \textbf{Fill the grid (small $\tau$).} Continue to propagate the values for small time differences $\tau=t-t'\ll1$. In terms of the algorithm it means that we have some elements of the grid, $N_c$ of them, close to the diagonal that will be updated by linear propagation because the approximation of small $\tau$ is still valid. In our simulation the first $\Delta t$ is of the order $10^{-7}$ and $N_c=2$. 
    \item \textbf{Fill the grid (larger $\tau$).} The rest of the values will be copied from the previous $t$ ($A_{t+\Delta t,t'}=A_{t,t'}$). These values are the initial guess for solving the self-consistent equations (\ref{eq:self-consistent algo 1}-\ref{eq:self-consistent algo 2}-\ref{eq:self-consistent algo 3}) and (\ref{eq:self-consistent algo mu}), in this procedure the derivatives are updated using the 2nd order discretization.
    \item \textbf{Half the grid and expand.} The grid is decimated which means that each observable is contracted $A_{i,j}\leftarrow A_{2i,2j}$ and the derivate are updated as follows $dA^{(h)}_{i,j}\leftarrow \frac12(dA^{(h)}_{2i,2j}+dA^{(h)}_{2i-1,2j})$, $dA^{(v)}_{i,j}\leftarrow \frac12(dA^{(v)}_{2i,2j}+dA^{(v)}_{2i,2j-1})$. The new time step is now: $\Delta t \leftarrow 2\Delta t$.
    \item \textbf{Start over from step 2}.
\end{enumerate}




\subsection{Numerical checks on the dynamical algorithm}

The dynamic-grid algorithm has been checked in a variety of ways.

\begin{figure}[H]
    \centering
    \subfigure[$p=3 \quad \Delta_2=1.01$]{
        \includegraphics[scale=.4]{img/{mu_2+3_1.0100}.pdf}
    }
    \subfigure[$p=3 \quad \Delta_2=1.05$]{
        \includegraphics[scale=.4]{img/{mu_2+3_1.0500}.pdf}
    }
    \centering
    \subfigure[$p=3 \quad \Delta_2=1.10$]{
        \includegraphics[scale=.4]{img/{mu_2+3_1.1000}.pdf}
    }
    \subfigure[$p=3 \quad \Delta_2=2.00$]{
        \includegraphics[scale=.4]{img/{mu_2+3_2.0000}.pdf}
    }
    \caption{Evolution of the correlation with the signal at fixed $\Delta_2$ for different $\Delta_p$. The dotted red line overlapping with other lines, is the same quantity evaluated using the fixed grid algorithm up to time $100$. We have started the LSE from an informative initial condition.}
    \label{fig:overlap evolution comparison}
\end{figure}

\paragraph{Cross-checking using the fixed-grid algorithm.} For short times the dynamical equations were solved using the fixed-grid algorithm and compared with the outcome of the dynamic-grid algorithm, obtaining the same results, see Fig.~\ref{fig:overlap evolution comparison}. In the figure we used the fixed-grid with $t_{\max} = 100$ and the $\Delta t = 6.25*10^{-3}$.    
 
    \paragraph{Same magnetization in the easy region. } In the impossible and easy regions, the overlap with the signal of both AMP and dynamic-grid integration, converges to the same value. In Fig.~\ref{fig:magnetization vs AMP} we show the overlap obtained with AMP, black dashed line, and the overlap achieved by the integration scheme at a given time. We can see that the overlap with the signal as obtained solving the LSE equations converges to the same value of the fixed point of AMP. Given a fixed $\Delta_2$ we can observe that the time to convergence increase very rapidly as we decrease $\Delta_p$. We fitted this increase of the \emph{relaxation time} to get the boundary of the Langevin hard region.

\begin{figure}[H]
    \centering
    \subfigure[$p=3 \quad \Delta_2=0.40$]{
        \includegraphics[scale=.48]{img/{m_convergence2AMP_2+3_0.4000}.pdf}
    }
    \subfigure[$p=3 \quad \Delta_2=0.60$]{
        \includegraphics[scale=.48]{img/{m_convergence2AMP_2+3_0.6000}.pdf}
    }
    \centering    
    \subfigure[$p=3 \quad \Delta_2=0.70$]{
        \includegraphics[scale=.48]{img/{m_convergence2AMP_2+3_0.7000}.pdf}
    }
    \subfigure[$p=3 \quad \Delta_2=0.80$]{
        \includegraphics[scale=.48]{img/{m_convergence2AMP_2+3_0.8000}.pdf}
    }
    \caption{Correlation with the signal of AMP (dotted lines) and Langevin (solid lines) at $k$th iteration and $t$ time respectively. The black dashed line is the asymptotic value predicted with AMP. In the easy region, provided enough running time, Langevin dynamics finds the same alignment as AMP. The figures show qualitatively the same behaviour for different values of $\Delta_2$.}
    \label{fig:magnetization vs AMP}
\end{figure}




\paragraph{Dynamical transition.}
The dynamical transition where the finite magnetization fixed point disappears can be regarded as a clustering or dynamical glass transition.
Indeed coming from the impossible phase, going towards the hard phase, at the dynamical transition the free energy landscape
changes and the unique ergodic paramagnetic minimum of the impossible phase gets clustered into an exponential number of metastable glassy states (see Sec. \ref{sec:replica analysis}).
Correspondingly the relaxation time of the Langevin algorithm diverges. Fitting this divergence with a power law we obtain an alternative estimation of the
dynamical line.  In the right panel of Fig.~\ref{fig:phase diagram p=3_all} we plot with yellow points the dynamical transition line as extracted from the fit of the relaxation
time of the Langevin algorithm extracted coming from the impossible phase and entering in the hard phase.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extrapolation procedure}

In order to determine the Langevin Hard region, given a fixed value of $\Delta_p$ ($\Delta_2$), we measure the relaxation time that it takes to relax to equilibrium. On approaching the Langevin hard region, this relaxation time increases and we extrapolate the divergence to obtain the critical $\Delta_p^*$ ($\Delta_2^*$ respectively) where the relaxation time diverges. The extrapolation is done assuming a power law divergence. Fig.~\ref{fig:phase diagram p=3_all} shows the results of this procedure for the cases $2+3$ and $2+4$.




\begin{figure}
    \centering
    \includegraphics[scale=.5]{img/PhaseDiagram_2+3_all_2.pdf}
        \includegraphics[scale=.5]{img/PhaseDiagram_2+4_all.pdf}
    \caption{On the left: phase diagram of the spiked matrix-tensor model for
      $p=3$ as presented in the left panel of Fig.~\ref{fig:phase diagram p=3} with the
      additional boundary of the Langevin hard phase (green circles and stars). 
      The boundary of the Langevin hard phase has been obtained by fitting the relaxation time at fixed $\Delta_p$ and increasing $\Delta_2$ (circles) and 
      conversely,  at fixed $\Delta_2$ and decreasing $\Delta_p$ (stars).
	 The blue dashed line
      marks a region above which we do not observe anymore a stable positive 1RSB complexity. 
      Finally we plot with orange and yellow dots the dynamical transition line as extracted from the relaxation time of the Langevin algorithm coming from respectively the hard and impossible phase.
      On the right: phase diagram of the spiked matrix-tensor model for
      $p=4$ as presented in the right panel of Fig.~\ref{fig:phase diagram p=3} with the additional Langevin hard phase boundary. Also in this case we observe that Langevin hard phase extends in the AMP easy phase. Interestingly the Langevin hard phase here folds and closes near the tri-critical point.  The blue dashed line
      marks a region above which we do not observe anymore a stable positive 1RSB complexity.
}    \label{fig:phase diagram p=3_all}
\end{figure}



\paragraph{Numerical checks on the extrapolation procedure.} 




To test
the quality of the fits we use a similar numerical procedure to locate the
spinodal of the informative solution, which is given by the points
where the informative solution ceases to exist. This spinodal
must be the same for both the AMP and the Langevin algorithm \cite{REVIEWFLOANDLENKA}. 

Since we aim at studying the spinodal of the informative solution, we initialize the LSE with $\Cmag_0=1$ and let it relax, measuring the time it takes to equilibrate at the value of $\Cmag$ given by the informative fixed point of AMP.
We do this fixing $\Delta_2$ and changing $\Delta_p$.
As we approach the critical $\Delta_{p,dyn}$, the relaxation time will diverge and we can fit this divergence with a power law. The dynamic threshold extracted in this way is finally compared with the one obtained from AMP. In Fig.~\ref{fig:fitDeltapSol} we show how this scheme has been applied for $\Delta_2\in\{1.01,\;1.05,\;1.10,\;2.00\}$. As we get closer to the critical line $\Delta_2=1$ the relaxation time increases (and the height of the plateau decreases), making the fit harder.
    All in all, we observe a very good agreement between the points found with these extrapolation procedures and the prediction obtaine with AMP, as shown in Fig.~\ref{fig:phase diagram p=3_all}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Annealing protocol}


In this section we show that using specific protocols we are able to enter in the Langevin hard region. 
A generic annealing scheme would lower the noises of both the channels simultaneously, which, as we tested and discussed in the main text, will not be able to avoid the Langevin hard region. Instead we can use the following protocol
\begin{equation}
	\begin{split}
		& T_2 \equiv 1 \, , \\ 
		& T_p \equiv T_p(t) = 1+\frac{C}{\Delta_p}e^{-\frac{t}{\tau_\text{ann}}} \ .
	\end{split}
\end{equation} 
The constant $C$ allows to select at the initial time the desired effective
$\Delta_{p,{\rm eff}}=\Delta_p+Ce^{-\frac{t}{\tau_\text{ann}}}$ far
from (and much larger than) the original one. Instead $\tau_\text{ann}$
chooses the speed of the annealing protocol. Fig.~\ref{fig:smartAnnealing}
shows that using this protocol we are able to enter in Langevin Hard
region even with $\Delta_2$ close to the AMP threshold. To this
purpose we initiated the effective $\Delta_{p,{\rm eff}}$ close to $100$ (i.e. $C=100$), very far from the Langevin hard region, and we used different speeds for the annealing of $\Delta_p$ (different colors in the figures). In the figures we can observe that approaching the $\Delta_2 = 1$ we need slower and slower protocols (larger and larger $\tau_\text{ann}$). The reason for this behavior is due to the fact that approaching $\Delta_2 = 1$ with $\Delta_p=100$ a longer time is required to gain a non trivial overlap with the solution. Evidence of this growing timescale at $\Delta_p=100$ is given in Fig.~\ref{fig:relaxationTimeDeltap100} where we show the relaxation time for magnetizing to the solution varying $\Delta_2$. In particular, we can observe that at $\Delta_2 = 0.70$ the relaxation time is of the order of $100$ time units. 

\begin{figure}
    \centering
    \subfigure[$\Delta_2=1.01$: estimation $0.82857$ (AMP $0.82719$)]{
       \includegraphics[scale=.57]{img/{Fit_jump_2+3_T1.0100}.pdf}
    }
    \subfigure[$\Delta_2=1.05$: estimation  $0.67447$ (AMP $0.67382$)]{
        \includegraphics[scale=.57]{img/{Fit_jump_2+3_T1.0500}.pdf}
    }
    \centering
\subfigure[$\Delta_2=1.10$: estimation $0.59104$ (AMP $0.59034$)]{
    \includegraphics[scale=.57]{img/{Fit_jump_2+3_T1.1000}.pdf}
	}
    \subfigure[$\Delta_2=2.00$: estimation  $0.34326$ (AMP $0.34314$)]{
        \includegraphics[scale=.57]{img/{Fit_jump_2+3_T2.0000}.pdf}
    }
    \caption{Relaxation time obtained from the LSE starting from an informative initial condition $\Cmag_0=1$. The four cases refers to the $2+3$ model and are fitted with a power law and the relaxation time appears to diverge very close to point predicted by AMP (the AMP prediction is given in the captions).} 
    \label{fig:fitDeltapSol}
\end{figure}

For the protocol to be successful it is therefore crucial that the
annealing time $\tau_{ann}$ is large enough to give the possibility of
magnetizing the solution before $\Delta_{p,{\rm eff}}$ has significantly decreased towards $\Delta_p$.
According to this analysis, it is not surprising that in Fig.~\ref{fig:smartAnnealing} for $\Delta_2=0.90$ the proposed protocol seems not to be successful. For this value of the parameter $\Delta_2$, the time to find a solution even with $\Delta_p=100$ should be larger than $1000$ time units, which is much larger than the used $\tau_{ann}$ and anyway out of the time window of our numerical solution. 
However, with an annealing time large enough it would be in principle possible to recover exactly the same boundaries of the AMP easy region. 

\begin{figure}
    \centering
    \subfigure[$\Delta_2=0.50$, $\Delta_p=0.10$]{
        \includegraphics[scale=.49]{img/{Policy_0.50_0.10}.pdf}
    }
    \subfigure[$\Delta_2=0.50$, $\Delta_p=0.20$]{
        \includegraphics[scale=.49]{img/{Policy_0.50_0.20}.pdf}
    }
    \subfigure[$\Delta_2=0.50$, $\Delta_p=0.30$]{
        \includegraphics[scale=.49]{img/{Policy_0.50_0.30}.pdf}
    }
    \centering
    \subfigure[$\Delta_2=0.70$, $\Delta_p=0.10$]{
        \includegraphics[scale=.49]{img/{Policy_0.70_0.10}.pdf}
    }
    \subfigure[$\Delta_2=0.70$, $\Delta_p=0.20$]{
        \includegraphics[scale=.49]{img/{Policy_0.70_0.20}.pdf}
    }
    \subfigure[$\Delta_2=0.70$, $\Delta_p=0.30$]{
        \includegraphics[scale=.49]{img/{Policy_0.70_0.30}.pdf}
    }
    \subfigure[$\Delta_2=0.90$, $\Delta_p=0.10$]{
        \includegraphics[scale=.49]{img/{Policy_0.90_0.10}.pdf}
    }
    \subfigure[$\Delta_2=0.90$, $\Delta_p=0.20$]{
        \includegraphics[scale=.49]{img/{Policy_0.90_0.20}.pdf}
    }
    \subfigure[$\Delta_2=0.90$, $\Delta_p=0.30$]{
        \includegraphics[scale=.49]{img/{Policy_0.90_0.30}.pdf}
    }
    \caption{The figures show the correlation with the signal in time obtained using different annealing protocols, whose details are reported in the legend of the first figure. All the protocols have $C=100$ which means that all the dynamics start with close effective $\Delta_p\sim100$, $T_p(0)\Delta_p\simeq100$. What changes among the different lines is the relaxation speed, from the fastest, drawn in blue, to the slowest, drown in brown. They are compared with the asymptotic value of AMP, dotted line, and the Langevin dynamics without smart annealing, dashed line.}
    \label{fig:smartAnnealing}
\end{figure}

\begin{figure}
	\centering
	\subfigure[]{
		\includegraphics[scale=.4]{img/{2+3_Tp100.0000_relaxation_time}.pdf}
	}
	\caption{Relaxation times of Langevin dynamics at $\Delta_p=100$ without using protocols starting from $\Cmag_0 = 10^{-4}$.}
	\label{fig:relaxationTimeDeltap100}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Glassy nature of the Langevin hard phase: the replica approach}\label{sec:replica analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we study the landscape of the spiked matrix-tensor problem following the approach of \cite{antenucci2018glassy}.
We underline here that we are interested in studying the free energy landscape problem rather than the energy landscape since
the former is the relevant quantity for finite temperatures ($\beta=1$ in our case, as discussed in Sec.~\ref{sec:model}). 
The results of \cite{antenucci2018glassy} suggest that the AMP-hard phase
and part of the AMP-easy phase are glassy. Therefore we could expect that low magnetization glassy states
trap the Langevin algorithm and forbid the relaxation to the equilibrium configurations that surrounds the signal.
This may happen also in a region where AMP instead is perfectly fine in producing configurations strongly correlated with the signal.
In order to check this hypothesis we compute the
logarithm of the number of glassy states, called the
complexity by using the replica method \cite{monasson1995structural, antenucci2018glassy}. 
The goal of this analysis is to trace an additional
line in the phase diagram that delimits the region where stable 
one step replica symmetry breaking (1RSB) metastable states
exist. We conjecture that this provides a physical lower bound to the Langevin hard phase 
in the $(\Delta_p, 1/\Delta_2)$ phase diagram.

\subsection{Computation of the complexity through the replica method}

The replica trick is based on the simple identity: $\mathbb{E}\log x =  \lim_{n\rightarrow0} \frac{\partial}{\partial n}\mathbb{E}x^n$.
Using this observation we can compute the expected value of the free
energy, $\Phi = - (\log Z)/N$, averaging the $Z^n$ and taking the limit
$n\rightarrow0$. This is in general as difficult as the initial
problem, however, if we consider only integer $n$ and extrapolate to
$0$, the computation becomes much less involved due to the fact that for integer $n$ the average $\mathbb{E}x^n$ can be sometimes performed analytically. 
Indeed in this case the
replicated partition function $Z^n$ can be regarded as the partition
function of $n$ identical uncoupled systems or replicas. Averaging over the disorder we obtain a clean system of interacting replicas.
The Hamiltonian of this system displays an emerging \emph{replica symmetry} since it is left unchanged by a permutation of replicas.
This symmetry can be spontaneously broken in certain disordered models where frustration is sufficiently strong \cite{MPV87}.

In mean field models characterized by fully connected factor graphs, the resulting Hamiltonian of interacting replicas
depends on the configuration of the system only through a simple order parameter, the overlap $\tilde Q$ between them, which is a $n\times n$ matrix that describes the similarities 
of the configurations of different replicas in phase space.
Furthermore the Hamiltonian is proportional to $N$ which means that in the thermodynamic limit $N\to \infty$, 
the model can be solved using the saddle point method. 
In this case one needs to consider a simple ansatz for the saddle point structure of the matrix $\tilde Q$ that allows to take the analytic continuation for $n\to 0$.
The solution to this problem comes from spin glass theory and general details can be found in \cite{MPV87}. 
The saddle point solutions for $\tilde Q$ can be classified according to the replica symmetry breaking level
going from the replica symmetric solution where replica symmetry is not spontaneously broken to various degree of spontaneous replica symmetry breaking
(including full-replica symmetry breaking). 
Here we will not review this subject but the interested reader can find details in \cite{MPV87}. 
The model we are analyzing can be studied in full generality at any degree of RSB (see for example \cite{CL04, CL06, CL13} where the same models have been studied in absence of a signal). 
However here we will limit ourselves to consider saddle point solutions up to a 1RSB level. 

The complexity of the landscape can be directly related to replica symmetry breaking. 
A replica symmetric solution implies an ergodic free energy landscape characterized by a single pure state.
When replica symmetry is broken instead, a large number of pure states arises and the phase space gets clustered in a hierarchical way \cite{MPV87}.
Making a 1RSB approximation means to look for a situation in which the hierarchical organization contains just one level: the phase space gets clustered into an 
exponential number of pure states with no further internal structure.

If we assume a 1RSB glassy landscape, we can compute the complexity of metastable states using a recipe due to Monasson \cite{monasson1995structural} (see also \cite{zamponi2010mean} for a pedagogical introduction).
The argument goes as follows. 

Let us consider system with $x$ \emph{real} replicas infinitesimally coupled. 
If the free energy landscape is clustered into an exponential number of metastable states, 
the replicated partition function, namely the partition function of the system of $x$ real replicas, can be written as  
$$ 
Z^x \simeq
e^{N[\Sigma(f^*)- x \beta f^*]} 
$$
where $f^*$ is the internal free energy of the dominant metastable states that is determined by the saddle point condition
$\frac{d\Sigma}{df}(f^*)= \beta x$ and $\beta$ the inverse temperature. Note that since we are interested in the Bayes optimal case, this corresponds to set $\beta=1$. 
The function $\Sigma(f)$ is the complexity of metastable states having internal entropy $f$.
Therefore, using the free parameter $x$ we can reconstruct the form of $\Sigma(f)$ from the replicated free energy.
In order to compute the replicated free energy we need to apply the
replica trick on the replicated system, $\overline{\log Z^x} =
\lim_{n\rightarrow0} \frac{\partial}{\partial n}\overline{(Z^x)^n}$. Calling the
replicated free energy $\Phi = -\frac1{N}\overline{\log Z^x}$, we get
the complexity as $\Sigma = x \frac{\partial\Phi}{\partial x}-\Phi$.

We can now specify the computation to our case where the partition function is the normalization of the posterior measure.
With simple manipulations of the equations \cite{CC05}, the partition function can be expressed as the integral over the overlap matrix
\begin{equation}
    \overline{(Z^x)^n} = \overline{Z_x^n} \propto \int \prod_{ab}dQ_{ab} e^{NnxS(Q)} \simeq \limsup_Q e^{NnxS(Q)}\,;
\end{equation}
where the overlap $Q$ is a $(nx+1)\times (nx+1)$ matrix 
\begin{equation*}
	Q = 
	\left(
	\begin{array}{c|c}
	  1 & m \cdots m \\ \hline
	  m & \raisebox{-15pt}{{\huge\mbox{$\tilde{Q}$}}} \\[-4ex]
	  \vdots & \\[-0.5ex]
	  m &
	\end{array}
	\right)
\end{equation*}
that contains a special row and column that encodes the overlap between different replicas with the signal
and therefore the corresponding overlap is the \emph{magnetization} $m$.


The 1RSB structure for the matrix $\tilde Q$ can be obtained by defining the following $nx\times nx$ matrices: the identity matrix $\mathbb{1}_{ij} = \delta_{ij}$, the full matrix $\mathbb{J}^{(0)}_{nx,ij} = 1$, and $\mathbb{J}_{nx}^{(1)} = \text{diag}(J_{x}^{(0)},\dots,J_{x}^{(0)})$ a block diagonal matrix where the diagonal blocks $J_{x}^{(0)}$ have size $x\times x$ and are matrices full of 1. In this case the 1RSB ansatz for $\tilde Q$ reads
\begin{equation*}
	\tilde{Q}=(1-q_M)\mathbb{1}_{nx}+(q_M-q_m)\mathbb{J}_{nx}^{(1)}+q_m\mathbb{J}_{nx}^{(0)}\,.
\end{equation*}
Using this ansatz we can compute $S(Q)$ that is given by
\begin{equation}\label{eq:1RSB action}
    \begin{split}
        S(Q) &= \frac1{nx}\left[\frac12\log\text{det}\;Q + \frac1{2p\Delta_p}\sum_{ab} Q_{ab}^p + \frac1{4\Delta_2}\sum_{ab} Q_{ab}^2\right]=\\
        &= \frac12\log(1-q_M)+\frac1{2x}\log\frac{1-q_M+x(q_M-q_m)}{1-q_M}+\frac12\frac{q_m-m^2}{1-q_M+x(q_M-q_m)}+\\
        &+ \frac1{2p\Delta_p}(1-q_M^p+x(q_M^p-q_m^p)+2m^p)+\frac1{4\Delta_2}(1-q_M^2+x(q_M^2-q_m^2)+2m^2)\,.
    \end{split}
\end{equation}
We can observe that starting from
this expression we can derive the RS free energy, \eqref{eq:free
  entropy generic}, taking $q_M =q_m$ or equivalently in the limit
$x\rightarrow1$.
From \eqref{eq:1RSB action} we obtain the saddle point equations
\begin{equation}\label{eq:Saddle Point complexity}
	\begin{split}
	    & 0 = 2\frac{\partial S}{\partial q_M} = (x-1)\left[\frac1x\left(\frac1{1-q_M+x(q_M-q_m)}-\frac1{1-q_M}\right)-\frac{q_m-m^2}{[1-q_M+x(q_M-q_m)]^2}+\frac{q_M^{p-1}}{\Delta_p}+\frac{q_M}{\Delta_2}\right]\,; \\
    	& 0 = 2\frac{\partial S}{\partial q_m} = x \left[\frac{q_m-m^2}{[1-q_M+x(q_M-q_m)]^2}-\frac{q_m^{p-1}}{\Delta_p}-\frac{q_m}{\Delta_2}\right]\,; \\
    	& 0 = \frac{\partial S}{\partial m} = \frac{-m}{1-q_M+x(q_M-q_m)}+\frac{m^{p-1}}{\Delta_p}+\frac{m}{\Delta_2}\,.
    \end{split}
\end{equation}
The low magnetization solution to these equations gives the complexity of the metastable branch of the posterior measure which is given by
\begin{equation}
    \begin{split}
        -\Sigma(x;Q^*) & = -\frac12\log\frac{1-q_M+x(q_M-q_m)}{1-q_M}+\frac{x}2\frac{q_M-q_m}{1-q_M+x(q_M-q_m)}-\frac{x^2}2\frac{(q_m-m^2)(q_M-q_m)}{[1-q_M+x(q_M-q_m)]^2}+\frac{x^2}2\frac{q_M^p-q_m^p}{p\Delta_p}+\\
        & +\frac{x^2}2\frac{q_M^2-q_m^2}{2\Delta_2}\,.
    \end{split}
\end{equation}
{\color{red}\textbf{Stefano:} there was a factor 1/2 in the RHS missing, check if the image is correct.}
The free parameter $x$ allows us to tune the free energy of the states
of which we compute the complexity. 
Thus we can characterize the part of the phase diagram where an exponential number of states is present.

To complete the 1RSB analysis we must compute the stability of the 1RSB saddle point solution for $Q$.
In particular it is important to compute the so called \emph{replicon} eigenvalues that characterizes the instability of this solution
towards further replica symmetry breaking.
Following \cite{crisanti1992sphericalp, CL13} we have two replicon eigenvalues given by
\begin{align}
	\label{eq:replicon I}
	\lambda_I &=
                    1-(1-q_M+x(q_M-q_m))^2\left[(p-1)\frac{q_m^{p-2}}{\Delta_p}+\frac1{\Delta_2}\right]\,
  ,\\
	\label{eq:replicon II}
	\lambda_{II} &=
                       1-(1-q_M)^2\left[(p-1)\frac{q_M^{p-2}}{\Delta_p}+\frac1{\Delta_2}\right]
                       \, .
\end{align}

\begin{figure}
    \centering
    \includegraphics[scale=.5,trim={0 0 0 1.401cm},clip]{img/{complexity_p3_Deltap0.50}.pdf}
    \caption{Complexity with as a function of the Parisi parameter $x$ for $p=3$ on the line $\Delta_p=0.5$. The solid line characterizes the stable part of the complexity while the dashed line the unstable one.}
    \label{fig:complexity p3 Deltap0.50}
\end{figure}


\begin{figure}
	\centering
	\subfigure[$p=3$; $\Delta_p = 0.50$; $\Delta_2 = 0.85$]{
		\includegraphics[scale=.4]{img/{complexity_f_p3_Delta20.85_Deltap0.50}.pdf}
	}
	\subfigure[$p=3$; $\Delta_p = 0.50$; $\Delta_2 = 0.90$]{
		\includegraphics[scale=.4]{img/{complexity_f_p3_Delta20.90_Deltap0.50}.pdf}
	}\\
	\subfigure[$p=3$; $\Delta_p = 0.50$; $\Delta_2 = 0.95$]{
		\includegraphics[scale=.4]{img/{complexity_f_p3_Delta20.95_Deltap0.50}.pdf}
	}
	\subfigure[$p=3$; $\Delta_p = 0.50$; $\Delta_2 = 1.00$]{
		\includegraphics[scale=.4]{img/{complexity_f_p3_Delta21.00_Deltap0.50}.pdf}
	}
	\caption{The stable part of the 1RSB complexity as
          a function of the free energy for $p=3$ and
          $\Delta_p=0.5$.}
	\label{fig:complexity f* p3 Deltap0.50}
\end{figure}


We can analyze what happens to the landscape when we fix $\Delta_p<1$ and we start from a large value of $\Delta_2<\Delta_{2,dyn}(\Delta_p)$ and we decrease $\Delta_2$.
In this case for sufficiently high $\Delta_2$ and large enough $\Delta_p$ the system is in a paramagnetic phase and no glassy states are present. 
At the dynamical transition line instead we find a positive complexity as plotted in Fig.~\ref{fig:complexity p3 Deltap0.50}. At this point the equilibrium states that dominate the posterior measure are the
so called \emph{threshold} states for which the complexity is maximal. For those states the eigenvalue $\lambda_{II}=0$ which confirms that these states are marginally stable \cite{cugliandolo1993analytical}.
Decreasing $\Delta_2$ one crosses the information theoretic phase transition where the relevant metastable states that dominate the posterior measure have zero complexity. 
This corresponds to a freezing/condensation/Kauzmann transition. Below the information theoretic phase transition the thermodynamics of the posterior measure is dominated
by the state containing the signal. However one can neglect the high magnetization solution of the 1RSB equations to get the properties of the metastable branch and computing the 
complexity of states that have zero overlap with the signal.
The complexity curves as a function of the Parisi parameter $x$ for decreasing values of $\Delta_2$ are plotted in Fig.~\ref{fig:complexity p3 Deltap0.50} for fixed $\Delta_p=0.5$ and several $\Delta_2$.
The curves contain a stable 1RSB part and an unstable one where $\lambda_{II}$ is negative.
The 1RSB line shown in Figs.~\ref{fig:phase diagram p=3_all} is obtained by looking at when the states with positive complexity and $\lambda_{II}=0$ disappear. 
This means that it gives the point where the 1RSB marginally stable states disappear and therefore it is expected to be a lower bound for the disappearance of glassiness in the phase diagram.
The important outcome of this analysis is that for $\Delta_2<1$ but not sufficiently small, namely in part of the AMP-easy phase, the replica analysis predicts the existence of 1RSB marginally stable glassy states that may trap the Langevin algorithm from relaxing towards the signal \cite{antenucci2018glassy}
and therefore supports the existence of the Langevin hard phase.

Finally in Fig.~\ref{fig:complexity f* p3 Deltap0.50} we plot the complexity as a function of the internal free energy of the metastable states for some values of $\Delta_2$ and $\Delta_p$. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Breakdown of the fluctuation-dissipation theorem in the Langevin hard phase}
When the Langevin algorithm is able to reach equilibrium, being it the signal or the paramagnetic state, it should satisfy the Fluctuation-Dissipation
Theorem (FDT) according to which the response function is related to the correlation function through $R(t,t') = -\frac{\partial C(t,t')}{\partial t}$.
Furthermore, time translational invariance (TTI) should arise implying that both correlation and response functions should be functions of only the time difference meaning that $R(t,t')=R(t-t')$ and $C(t,t')=C(t-t')$\footnote{All one time quantities are constant in equilibrium.}.
When the dynamics is run in the glass phase, metastable states may forbid equilibration.
In this case time translational invariance is never reached at long times\footnote{It is supposed to be reached only on exponential timescales in the system size.} and the dynamics displays aging violating at the same time the FDT relation.
The analysis of the asymptotic aging dynamics has been cracked by Cugliandolo and Kurchan in \cite{cugliandolo1993analytical, CK95} (see also \cite{Cu03} for a pedagogical review) in the simplest spin glass model (see also \cite{CK94SK} for a much more complex situation) where no signal is present. 
The outcome of this work is that when the dynamics started from a random initial conditions is run in the glass phase, it drives the system to surf on the \emph{threshold} states.
In the model analyzed in \cite{cugliandolo1993analytical} these states correspond to the 1RSB marginally stable glassy states that maximize the complexity.
In this section we analyze the Cugliandolo-Kurchan scenario by contrasting the numerical solution of the dynamical equations with the replica analysis of the complexity.
According to \cite{cugliandolo1993analytical}, the long time Langevin dynamics\footnote{But still for times that are not exponentially large in the system size $N$.}
can be characterized by two time regimes. 
For short times differences $t-t'\sim {\cal O}(1)$ and $t'\to \infty$, the system obeys the FDT theorem and TTI; this regime can be understood as a first fast local equilibration in the nearest metastable state available.
On a longer timescale $t-t'\to \infty$ and $t/t'<\infty$, the dynamics surfs on threshold states and FDT and TTI are both violated.
In this time window, both the response and correlation functions become functions of $\lambda=h(t)/h(t')$ being $h(t)$ an arbitrary reparametrization of the time variable\footnote{The function $h(t)$ must be a monotonously increasing function. The asymptotic reparametrization invariance is a key property of the dynamical equations \cite{cugliandolo1993analytical}.}. By defining ${\cal C(\lambda)} = C(t,t')$ and ${\cal R(\lambda)} = tR(t,t') $ the Cugliandolo-Kurchan solution implies that in this aging regime the FDT relation can be generalized to
\begin{equation}
	\label{eq:generalized FDT}
	\mathcal{R}\left(\lambda\right) = x\    \mathcal{C}'\left(\lambda\right)
\end{equation}
with $x$ an \emph{effective} FDT ratio that controls how much the FDT is violated. 
In the scenario of \cite{cugliandolo1993analytical}, the value of $x$ coincides with the 1RSB Parisi parameter that corresponds to threshold states computed within the replica approach.
In order to test this picture we follow Cugliandolo and Kurchan \cite{CK97} and we plot the integrated response ${\cal {F}}(t,t') = -\int_{t'}^t R(t,t'')dt''$ as a function of $C(t,t')$ in a parametric way.
This is done in Fig.~\ref{fig:generalized FDT fit}.


If FDT holds at all timescales, one should see a straight line with slope $-1$. 
Instead what we see in the Langevin hard phase is that for large values of $t'$ the curves approach asymptotically for $t'\gg 1$ two straight lines. 
For high values of $\cal C$, meaning for short time differences $t-t'\sim {\cal O}(1)$, the slope of the straight line is $-1$ which means that ${\cal F}=1-{\cal C}$ as implied by the short time FDT relation.
On longer timescales FDT is violated, confirming the glassiness of the Langevin hard phase.
By doing a linear fit we can use the data plotted in Fig.~\ref{fig:generalized FDT fit} to estimate the FDT ratio $x$ appearing in Eq.~(\ref{eq:generalized FDT}). This can be compared with the Parisi parameter $x$ for which we have marginally stable 1RSB states.
We find an overall very good agreement (data coming from the fit is reported in the caption of Fig.~\ref{fig:generalized FDT fit}).
The small discrepancy between the two values of $x$ can be either due to the numerical accuracy in solving the dynamical equations as well as the possibility that the 1RSB threshold is not exactly the one that characterizes the long time dynamics. Further investigations are needed to clarify this point.  
Finally, according to \cite{cugliandolo1993analytical} the value of $\cal C$ at which the two straight line cross should coincide with the value of $q_M$ computed for the threshold states within the 1RSB solution.
Again we find a very good agreement. 

\begin{figure}
	\centering
    \subfigure{
        \includegraphics[scale=.6]{img/{FDT_2+3_T0.8000_Tp0.2000}.pdf}
      	\includegraphics[scale=.6]{img/{FDT_2+3_T1.4000_Tp0.2000}.pdf}
    }
    \caption{Left panel: parametric plot of integrate response function with
      respect to correlation function for $p=3$, $\Delta_2 = 0.8$ and
      $\Delta_p = 0.2$. The different lines represent different
      waiting time, $t'$. The black dashed line correspond to the FDT prediction
      $x=1$. The vertical dotted line is the point where we
      observe a kink, which we denote by 
      ${\cal C}=\hat q_{EA}$ and should be equal to the saddle point value of $q_M$ as extracted from the 1RSB threshold states in the replica computation \cite{cugliandolo1993analytical}:
      $\hat q_{EA} = 0.633$ and $q_M = 0.638$. For $\mathcal{C}$
      smaller than $q_{EA}$ the FDT is violated and is replaced by a generalized version as in Eq.~(\ref{eq:generalized FDT}). We can
      obtain the value of the FDT ratio from a fit of the slope of the asymptotic curves for ${\cal C}<\hat q_{EA}$.
      We obtain $\hat x = 0.397$ which should be compared with the Parisi
      parameter that corresponds to 1RSB marginally stable states obtained from the replica computation that is $x = 0.408$.
      Right panel:  parametric plot of the integrated response as a function of the correlation
      for $p=3$ and $\Delta_2=1.4$ and $\Delta_p=0.2$. In this case the value of the FDT ratio
      extracted from fitting the data is $\hat x=0.397$ to be compared with the value of the Parisi parameter for the 1RSB threshold states that is $x=0.408$.
      At the same time data gives $\hat q_{EA}=0.633$ while the replica computation gives $q_M =0.638$.
          }
    \label{fig:generalized FDT fit}
\end{figure}




%\begin{figure}
%	\centering
%    \subfigure[$p=3 \quad \Delta_p=0.20$]{
%        \includegraphics[scale=.5,trim={0 0 0 .592cm},clip]{img/{2+3_x_0.2}.pdf}
%    }
%    \subfigure[$p=3 \quad \Delta_p=0.30$]{
%        \includegraphics[scale=.5,trim={0 0 0 .592cm},clip]{img/{2+3_x_0.3}.pdf}
%    }
%    \subfigure[$p=3 \quad \Delta_p=0.40$]{
%        \includegraphics[scale=.5,trim={0 0 0 .592cm},clip]{img/{2+3_x_0.4}.pdf}
%    }
%    \subfigure[$p=3 \quad \Delta_p=0.50$]{
%        \includegraphics[scale=.5,trim={0 0 0 .592cm},clip]{img/{2+3_x_0.5}.pdf}
%    }
%    \caption{Fitted value of the parameter of violation of FDT for different waiting times $t_w$. Different lines and figures represent different regions of the phase space, i.e. different values of $\Delta_2$ and $\Delta_p$. The values is compared with the Parisi parameter obtained by the marginal stability condition (dotted line).} 
%    \label{fig:generalized FDT evolution}
%\end{figure}



